LL-GNN: Low Latency Graph Neural Networks on FPGAs for High Energy Physics

This work presents a novel reconfigurable architecture for Low Latency Graph Neural Network (LL-GNN) designs for particle detectors, delivering unprecedented low latency performance. Incorporating FPGA-based GNNs into particle detectors presents a unique challenge since it requires sub-microsecond latency to deploy the networks for online event selection with a data rate of hundreds of terabytes per second in the Level-1 triggers at the CERN Large Hadron Collider experiments. This paper proposes a novel outer-product based matrix multiplication approach, which is enhanced by exploiting the structured adjacency matrix and a column-major data layout. Moreover, a fusion step is introduced to further reduce the end-to-end design latency by eliminating unnecessary boundaries. Furthermore, a GNN-specific algorithm-hardware co-design approach is presented which not only finds a design with a much better latency but also finds a high accuracy design under given latency constraints. To facilitate this, a customizable template for this low latency GNN hardware architecture has been designed and open-sourced, which enables the generation of low-latency FPGA designs with efficient resource utilization using a high-level synthesis tool. Evaluation results show that our FPGA implementation is up to 9.0 times faster and achieves up to 13.1 times higher power efficiency than a GPU implementation. Compared to the previous FPGA implementations, this work achieves 6.51 to 16.7 times lower latency. Moreover, the latency of our FPGA design is sufficiently low to enable deployment of GNNs in a sub-microsecond, real-time collider trigger system, enabling it to benefit from improved accuracy. The proposed LL-GNN design advances the next generation of trigger systems by enabling sophisticated algorithms to process experimental data efficiently.

==> algo_reviewer3.tex <==
\begin{algorithm}[t]
  \caption{Code transformation with an FSM to transfer an imperfect loop into a perfect loop.}
  \label{algo:loop_fusion_reviewer}
  \LinesNumbered
  


\For{$i = 0$ to $N_o$}{ 
%\For{$ik = 0$ to $N_o \times (N_o-1)$}{ 
%\textcolor{blue}{ \#pragma HLS PIPELINE }\\

%        $i = int(\frac{ik}{N_o-1})$; \\
%        $k = ik\%(N_o-1)$; \\
    \For{$k = 0$ to $N_o-1$    } { 
        \textcolor{blue}{  \#pragma HLS PIPELINE  }\\
        \textcolor{blue}{  \#pragma HLS UNROLL factor$=N_{fR}$  }\\

       % \textcolor{blue}{ \#pragma HLS PIPELINE} \\
        \textcolor{ForestGreen}{ code\_body\_A;}\\
        \If{$k == (N_o-2)$}
        {
            \textcolor{ForestGreen}{code\_body\_B;} \\
        }
    }

}



\end{algorithm}

==> cmp_cpugpu_t.tex <==
\begin{table}[t]
\centering

\caption{Comparison of the FPGA, CPU and GPU designs.}
\label{tab:cmp_cpugpu}
\begin{threeparttable}
\centering
\scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c}
\toprule

% & \multicolumn{2}{c|}{\cite{moreno2020jedi}} & \multicolumn{3}{c}{This work} \\ 
%\midrule
Platform
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} CPU \\Gold 6154\end{tabular}}
%& \multicolumn{2}{c|}{GPU GeForce 2080Ti}
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} GPU \\GeForce 2080Ti\end{tabular}}


& \multicolumn{2}{c}{FPGA U250}
%& \begin{tabular}[c]{@{}c@{}}CPU \\ E2620 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}GPU \\ TITAN X \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}FPGA \\ U250 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}Zynq\\ 7Z045 \end{tabular} 
\\ \midrule

Frequency 
&\multicolumn{2}{c|}{3.00 GHz}
&\multicolumn{2}{c|}{1.63 GHz}
&\multicolumn{2}{c}{200 MHz}
\\
%Frequency & 3.4 GHz & 1.62 & 3.4 GHz & 1.62 & 200 MHz \\ 
\midrule
Technology 
&\multicolumn{2}{c|}{14 nm}
&\multicolumn{2}{c|}{12 nm}
&\multicolumn{2}{c}{28 nm}
\\ \midrule
Precision 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c}{24 Fixed}   
\\ 
%\midrule
%NN Model& \multicolumn{4}{c}{ JEDI-net-30p } \\
\midrule
%\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net\end{tabular}
%& 50p & 30p &  50p &30p  & 50p &  30p\\

\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} \cite{moreno2020jedi, que2022optimizing} \\  50p \end{tabular}
%& \begin{tabular}[c]{@{}c@{}} \cite{moreno2020jedi, que2022optimizing} \\ 30p \end{tabular}

& 50p\tnote{1} & 30p\tnote{1} 
&  50p\tnote{1} &30p\tnote{1}  

& 50p &  30p\\

\midrule
Power (W) &103  &106  & 250  & 245 & 25.9   & 24.0\\ 
\midrule
Batch Size & \multicolumn{6}{c}{1000} \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Average Lat.\\($\mu$s) \end{tabular}
  &593.1  &56.9  & 16.8 & 3.8 & 0.75 & 0.75 \\ 
%\midrule
%Energy (mJ) & 2.156 & 1.584 & 0.012  \\   
\midrule
\begin{tabular}[c]{@{}c@{}}Throughput\\ (KGPS) \end{tabular} 
 & 1.69   &17.6 &  59.52 & 263.2  & 1333  & 1333\\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Power Effic.\\ (KGPS/W) \end{tabular} &0.02  &0.17  & 0.24 & 1.07   & 51.5 &  55.5\\ 
\midrule
\end{tabular} }
   \begin{tablenotes}
    \footnotesize
        \item[1] Same JEDI-net architecture to~\cite{moreno2020jedi, que2022optimizing}.
    \normalsize
   \end{tablenotes}
\end{threeparttable}

\end{table}

==> cmp_cpugpu_t2.tex <==
\begin{table}[t]
\centering

\caption{\textcolor{\mycolor}{Comparison of the FPGA, CPU and GPU designs.}}
\label{tab:cmp_cpugpu}
\begin{threeparttable}
\centering
\scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c}
\toprule

% & \multicolumn{2}{c|}{\cite{moreno2020jedi}} & \multicolumn{3}{c}{This work} \\ 
%\midrule
Platform
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} CPU \\Gold 6154\end{tabular}}
%& \multicolumn{2}{c|}{GPU GeForce 2080Ti}
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} GPU \\GeForce 2080Ti\end{tabular}}

& \multicolumn{2}{c}{FPGA U250}
%& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}  FPGA U250 \\ (This work)\end{tabular}}
%& \begin{tabular}[c]{@{}c@{}}CPU \\ E2620 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}GPU \\ TITAN X \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}FPGA \\ U250 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}Zynq\\ 7Z045 \end{tabular} 
\\ \midrule

Frequency 
&\multicolumn{2}{c|}{3.00 GHz}
&\multicolumn{2}{c|}{1.63 GHz}
&\multicolumn{2}{c}{200 MHz}
\\
%Frequency & 3.4 GHz & 1.62 & 3.4 GHz & 1.62 & 200 MHz \\ 
\midrule
Technology 
&\multicolumn{2}{c|}{14 nm}
&\multicolumn{2}{c|}{12 nm}
&\multicolumn{2}{c}{28 nm}
\\ \midrule
Precision 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c}{24 Fixed}   
\\ 
%\midrule
%NN Model& \multicolumn{4}{c}{ JEDI-net-30p } \\
\midrule
%\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net\end{tabular}
%& 50p & 30p &  50p &30p  & 50p &  30p\\

\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net \end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
& 50p\tnote{1} & 30p\tnote{1} 
& 50p\tnote{1} & 30p\tnote{1} 
& \begin{tabular}[c]{@{}c@{}}50p\\ \textcolor{\mycolor}{( U4 )} \end{tabular}
& \begin{tabular}[c]{@{}c@{}}30p\\ \textcolor{\mycolor}{( J4 )} \end{tabular}
%50p (U4) &  (J4)
\\

\midrule
\textcolor{\mycolor}{Accuracy (\%)} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
\\ 

\midrule
Power (W) 
& \textcolor{\mycolor}{106}  
& \textcolor{\mycolor}{112}  
& \textcolor{\mycolor}{223}
& \textcolor{\mycolor}{225}
& \textcolor{\mycolor}{26.3}   
& \textcolor{\mycolor}{33.1}
\\ 
\midrule
Batch Size & \multicolumn{6}{c}{1000} \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Average Lat.\\($\mu$s) \end{tabular}
& \textcolor{\mycolor}{272.4}
& \textcolor{\mycolor}{42.3}  
& \textcolor{\mycolor}{6}
& \textcolor{\mycolor}{1.6} 
& \textcolor{\mycolor}{0.75} 
& \textcolor{\mycolor}{0.15} \\ 
%\midrule
%Energy (mJ) & 2.156 & 1.584 & 0.012  \\   
\midrule
\begin{tabular}[c]{@{}c@{}}Throughput\\ (KGPS) \end{tabular} 
 & \textcolor{\mycolor}{3.7}   
 & \textcolor{\mycolor}{23.6} 
 & \textcolor{\mycolor}{166.7}
 & \textcolor{\mycolor}{625.0}  
 & \textcolor{\mycolor}{1333}   
 & \textcolor{\mycolor}{6667} \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Power Effic.\\ (KGPS/W) \end{tabular} 
& \textcolor{\mycolor}{0.03}  
& \textcolor{\mycolor}{0.21}  
& \textcolor{\mycolor}{0.75} 
& \textcolor{\mycolor}{2.78}   
& \textcolor{\mycolor}{50.7} 
& \textcolor{\mycolor}{201.4} \\ 
\midrule
\end{tabular} }
   \begin{tablenotes}
    \footnotesize
        \item[1] \textcolor{\mycolor}{Same JEDI-net architecture to U4 or J4.}
    \normalsize
   \end{tablenotes}
\end{threeparttable}

\end{table}

==> cmp_cpugpu_t3.tex <==
\begin{table}[t]
\centering

\caption{\textcolor{\mycolor}{Comparison of the FPGA, CPU and GPU designs.}}
\label{tab:cmp_cpugpu}
\begin{threeparttable}
\centering
\scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|c}
\toprule

% & \multicolumn{2}{c|}{\cite{moreno2020jedi}} & \multicolumn{3}{c}{This work} \\ 
%\midrule
Platform
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} CPU \\Gold 6154\end{tabular}}
%& \multicolumn{2}{c|}{GPU GeForce 2080Ti}
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}} GPU \\\textcolor{\mycolor}{GeForce 3090}\end{tabular}}

& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} FPGA \\ U250\end{tabular} }
%& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}  FPGA U250 \\ (This work)\end{tabular}}
%& \begin{tabular}[c]{@{}c@{}}CPU \\ E2620 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}GPU \\ TITAN X \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}FPGA \\ U250 \end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}Zynq\\ 7Z045 \end{tabular} 
\\ \midrule

Frequency 
&\multicolumn{2}{c|}{3.00 GHz}
&\multicolumn{2}{c|}{\textcolor{\mycolor}{1.70 GHz}}
&\multicolumn{2}{c}{200 MHz}
\\
%Frequency & 3.4 GHz & 1.62 & 3.4 GHz & 1.62 & 200 MHz \\ 
\midrule
Technology 
&\multicolumn{2}{c|}{14 nm}
&\multicolumn{2}{c|}{\textcolor{\mycolor}{8 nm}}
&\multicolumn{2}{c}{16 nm}
\\ \midrule
Precision 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c|}{F32} 
&\multicolumn{2}{c}{24 Fixed}   
\\ 
%\midrule
%NN Model& \multicolumn{4}{c}{ JEDI-net-30p } \\
\midrule
%\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net\end{tabular}
%& 50p & 30p &  50p &30p  & 50p &  30p\\

\begin{tabular}[c]{@{}c@{}}NN Model\\JEDI-net \end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 50p \\(U4)\end{tabular}
%& \begin{tabular}[c]{@{}c@{}} 30p \\(J4)\end{tabular}
& 50p\tnote{1} & 30p\tnote{1} 
& 50p\tnote{1} & 30p\tnote{1} 
& \begin{tabular}[c]{@{}c@{}}50p\\ \textcolor{\mycolor}{( U4 )} \end{tabular}
& \begin{tabular}[c]{@{}c@{}}30p\\ \textcolor{\mycolor}{( J4 )} \end{tabular}
%50p (U4) &  (J4)
\\

\midrule
\textcolor{\mycolor}{Accuracy (\%)} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
& \textcolor{\mycolor}{80.90}  
& \textcolor{\mycolor}{78.41} 
\\ 

\midrule
Power (W) 
& \textcolor{\mycolor}{106}  
& \textcolor{\mycolor}{112}  
& \textcolor{\mycolor}{325}
& \textcolor{\mycolor}{326}
& \textcolor{\mycolor}{26.3}   
& \textcolor{\mycolor}{33.1}
\\ 
\midrule
Batch Size & \multicolumn{6}{c}{1000} \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Average Lat.\\($\mu$s) \end{tabular}
& \textcolor{\mycolor}{272.4}
& \textcolor{\mycolor}{42.3}  
& \textcolor{\mycolor}{4.5}
& \textcolor{\mycolor}{1.3} 
& \textcolor{\mycolor}{0.50} 
& \textcolor{\mycolor}{0.15} \\ 
%\midrule
%Energy (mJ) & 2.156 & 1.584 & 0.012  \\   
\midrule
\begin{tabular}[c]{@{}c@{}}Throughput\\ (KGPS) \end{tabular} 
 & \textcolor{\mycolor}{3.7}   
 & \textcolor{\mycolor}{23.6} 
 & \textcolor{\mycolor}{222.2}
 & \textcolor{\mycolor}{769.2}  
 & \textcolor{\mycolor}{2000}   
 & \textcolor{\mycolor}{6667} \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}Power Effic.\\ (KGPS/W) \end{tabular} 
& \textcolor{\mycolor}{0.03}  
& \textcolor{\mycolor}{0.21}  
& \textcolor{\mycolor}{0.68} 
& \textcolor{\mycolor}{2.36}   
& \textcolor{\mycolor}{76.0} 
& \textcolor{\mycolor}{201.4} \\ 
\midrule
\end{tabular} }
   \begin{tablenotes}
    \footnotesize
        \item[1] \textcolor{\mycolor}{Same JEDI-net architecture to U4 or J4.}
    \normalsize
   \end{tablenotes}
\end{threeparttable}

\end{table}

==> mainbody-old.tex <==



\section{Introduction}\label{subsec:introduction}



Recurrent Neural Network (RNN) has been the key component of artificial intelligence (AI) applications where the inputs are sequential, such as natural language processing~\cite{goldberg2016primer}, speech recognition~\cite{amodei2016deep, han2017ese} and video analysis~\cite{yue2015beyond, lrcn_donahue2015long}. 
Long Short-Term Memory (LSTM) is the most popular type of RNNs. Since low latency is key for a seamless user experience in such applications, efficient and real-time acceleration of RNNs/LSTMs is required. 
FPGAs have been used to speed up the inference of LSTMs \cite{nurvitadhi2016accelerating, guan2017fpga, sun2018fpga, fowers2018configurable, eriko_fccm19}, showing the benefits of low latency and low power consumption compared to CPUs or GPUs. 


However, existing RNN/LSTM accelerators cannot support cost-effective multi-RNN execution. Cloud providers must minimize their huge operation costs by running as many applications on a given server as possible, while satisfying the quality of each service. In Google data centers, CNNs (Convolutional Neural Networks) and MLPs (Multi-Layer Perceptions) comprise 5\% and 61\% of the workload respectively, while LSTMs makes up 29\%~\cite{jouppi2017datacenter}. However, most of the existing LSTM accelerators are only able to perform one inference at a time~\cite{mittal2021survey, fowers2018configurable, eriko_fccm19, que2020optimizing, han2017ese,guan2017fpga}. These accelerators can process multi-LSTM tasks by executing one by one in sequence, resulting in inefficiency when multiple requests come at the same time as shown in~\figref{fig:multi_task}. It may make later tasks wait for a long time before a hardware core is available, since earlier LSTM tasks may have a large number of timesteps involving many iterations, e.g., an LSTM layer in DeepSpeech~\cite{deepspeech} has 1500 timesteps. 
Besides, some applications employ not one, but multiple LSTMs to collaboratively achieve satisfactory performance. A spacecraft anomalies detection system~\cite{hundman2018detecting} even contains over hundreds of LSTM models, each modeling a single telemetry channel and predicting values for that channel, which demonstrates the necessity of supporting multi-LSTM execution. 
Furthermore, conventional LSTM accelerators are often implemented by deploying all computing resources to support a single computational engine on a large scale, leveraging data-level parallelism. 
For instance, Brainwave~\cite{fowers2018configurable} devised by Microsoft is a single-threaded neural processing unit (NPU) which involves 96,000 processing elements (PEs). 
However, when the workload of a targeted LSTM task is small, these hardware resources will not be fully utilized, e.g., the hardware utilization is lower than 1\%~\cite{fowers2018configurable} for Brainwave and lower than 15\% for the Brainwave-like NPU~\cite{eriko_fccm19} when running an LSTM model ($h_t$=256). It is challenging to design an accelerator to support cost-effective multi-LSTM execution.  

%there could be potential for workloads that see under-utilization of the pipeline using single-thread

\begin{figure}[b]
\begin{center}
\includegraphics[width=0.90\linewidth]{img/multi_task_t03.pdf}
\end{center}
   \caption{Timeline of three LSTM inference tasks based on a first-come first-serve scheduling policy. The example of the LSTM-1 has two timesteps (TS), the LSTM-2 has three timesteps and the LSTM-3 has two timesteps in this figure.}
\label{fig:multi_task}
\end{figure}



%This paper proposes a reconfigurable multi-threaded multi-core neural processing unit (NPU) for accelerating LSTM inferences, which increases the processing abilities of cloud-based NPUs with high Quality of Service~(QoS) and improves hardware utilization for better performance. 
%This paper proposes a reconfigurable multi-threaded multi-core neural processing unit (NPU) to accelerate LSTM inferences so that the processing abilities of cloud-based NPUs with high Quality of Service~(QoS) can be increased and hardware utilization can be improved for better performance. 
This paper introduces a reconfigurable multi-threaded multi-core neural processing unit (NPU) for accelerating RNN/LSTM inferences by increasing the hardware utilization for better performance. It improves the processing abilities of cloud based NPUs as well as the Quality of Service~(QoS). 
Our primary goal is to efficiently enhance the scalability potential of NPU cores. The most area~/~cost efficient way to add logical cores is multithreading. Essentially, multithreading retrieves unused performance (where computational cores are idle because of events) by switching to another thread. Multithreading also does not affect peak performance when working in a single-threaded mode. 
Usually, the execution of multiple neural networks has the potential to mitigate the idle issues because layers from different neural networks can be scheduled freely without any issue of dependencies. 
Running multiple tasks can also be realized by batch techniques that provide multiple requests to a neural network to produce multiple results together. 
However, the batch techniques can harm latency because different requests may not arrive at the same time~\cite{gao2018low}, which means that a newly arrived request must wait until the batch is formed, 
%for an ongoing batch of requests to finish their execution completely, 
which brings a significant latency penalty as shown in~\figref{fig:batching}.  %Also, for inputs with different sizes, 

%t  harms  latency  because  different  inputs  do  not  come  atthe  same  time.  Also,  for  inputs  with  different  sizes,  in  thecombined  graph,  all  operators  cannot  be  fully  batched  andthus, improvement in throughput remains s
%Multiple execution of many inputs is straight forward when their underlying computation is  identical,  as  is  the  case  withMLPs  and  CNNs.  By  contrast,  as  inputs  affect  the  depth  ofrecursion, batching RNN computation is challen

Remarn is inspired by coarse-grained multithreading utilized in modern CPUs such as IBM RS64-IV~\cite{borkenhagen2000multithreaded} and Intel Montecito~\cite{mcnairy2005montecito}, which makes a core switch to a different hardware context when a thread is stalled due to some events. Remarn consists of a custom coarse-grained multi-threaded (CGMT) LSTM hardware architecture which switches tasks among threads when LSTM computational engines meet data hazard. 
When one logical NPU core is stalled, the other can make progress. Coarse-grained multithreading is a mature technique in modern CPU designs. However, few studies concern combining the CGMT and NPUs, especially for RNNs/LSTMs. There is also fine-grained multi-threading~\cite{thornton1964parallel, smith1986pipelined} which switches the context every cycle but it brings more hardware complexity than CGMT. 
Unlike CNNs that do not have memory cells and can run different layers from different neural networks iteratively, RNNs/LSTMs contains many memory cells, which makes it difficult to process different timesteps from different RNN layers or models since they have different cell memory statuses when using a single-threaded NPU. It has to finish the running of the preceding RNN inference or layer until the next inference or layer can start. 
%The inter-timestep dependencies within an RNN layer prevent the following timestep computation from even starting until the current timestep’s completion,
The existence of inter-timestep dependencies within an RNN model prevents the following timesteps from even starting their execution until the current timestep’s completion, leading to hardware underutilization and inefficiency. To address this challenge, this work proposes the CGMT-LSTM which can intelligently switch to an alternate thread of computation when the data hazard happens, e.g., the inter-timestep dependencies of RNNs, to increase hardware utilization and boost design performance. 

%The fine-grained multi-threading switches the context every cycle while the coarse-grained only switches the context when there is an event. 

%Compared with a fine-grained multithreading scheme 



\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.80\linewidth]{img/multi_task_batch_t02.pdf}
\end{center}
   \caption{Timeline of three LSTM inference tasks using a batching technique.}
\label{fig:batching}
\end{figure}



Besides, instead of deploying all computing resources to form a single physical core on a large scale like Brainwave~\cite{fowers2018configurable} and our previous design~\cite{que2020reconfigurable}, we design an accelerator hardware architecture which can be partitioned into multiple full-fledged sub-accelerator cores, and each core can accept new RNN requests. 
The multiple LSTM models used in the application of spacecraft anomaly detection system~\cite{hundman2018detecting} have only a small hidden vector size which is less than 128, but they have 250 timesteps which are large. LSTM models that have a large number of timesteps but utilize a small size are the most tangible examples since they require dealing with lots of dependencies, as well as the parallel task of matrix-vector multiplications (MVMs)~\cite{yazdani2019lstm}. The Brainwave~\cite{fowers2018configurable} involves big MVM ``tile engines" which can effectively process a $400\times 240$ matrix in parallel. Besides, our previous NPU~\cite{que2020reconfigurable} is based on a tile size of $1024\times 16$, resulting in 16,384 effective PEs. Any MVM that does not map to this dimension will leave some resources idle and small MVMs even require zero paddings, resulting in low utilization. Splitting a large accelerator into several small sub-accelerator cores can not only help to find a better mapping to improve hardware utilization but also provide more physical cores to spatially co-locate multiple RNN inferences on the same hardware.
As~\cite{fowers2018configurable} mentions, RNN programs have a critical loop-carry dependence on the $h_t$ vector. If the full pipeline cannot return $h_t$ to the vector register file in time for the next timestep computation, the MVM unit will stall until $h_t$ is available. 
%There is data hazard in RNN computation since the new hidden vector h_t$ is required for the next timestep computation. 
Thus, even if a large MVM engine finishes the LSTM gates operations in a short period, e.g., 1 cycle, the design still needs to wait for the $h_t$ returned from the pipeline, which shows the limitation of the architecture using a large engine. 
This work splits the accelerator with a single large engine into several smaller sub-accelerator cores, each of them processing small LSTM models more efficiently by adopting the tiling-based column-wise MVM approach~\cite{que2020optimizing}. It addresses the challenge of accelerating a large number of small LSTM models with large timesteps. Please note that these sub-accelerator cores can work together as a single large accelerator when necessary to deal with the high priority workloads which require the lowest end to end latency. 



%involves six matrix-vector multiplication (MVM) ``tile engines", each processing $400\times 40$ matrices. The results of the tile engine are then fed to a balanced adder-tree, so these engines can effectively process a $400\times 240$ matrix in parallel. Any MVM that does not map to this dimension will leave some resources idle.


%f-CNN$^x$~\cite{venieris2018f} proposes multiple custom dedicated CNN engines for the workloads with various CNN models. HDAs~\cite{kwon2021heterogeneous} are heterogeneous dataflow accelerators, which are composed of multiple sub-accelerators with different hardware architectures of dataflow, to support spatial co-executing multi-tenant workloads. Planaria~\cite{ghodrati2020planaria} is propsed to dynamically fission the DNN accelerator at runtime to spatially co-locate multiple DNN inferences on the same systolic array.

%Moreover, this work also introduces a hardware architecture which can be split into multiple sub-accelerators. It enables spatially co-executing multiple RNN/LSTM inferences on the same hardware and offers simultaneous multi-tenant RNN accelerations.



To the best of our knowledge, Remarn is the first coarse-grained multi-threaded and multi-core LSTM accelerator architecture capable of achieving high performance and efficient multi-LSTM execution.
%Challenges:
%1) Low hardware utilization since there is data dependence in the RNN.
%2) Inefficient DSP usage, especially for Xilinx DSP block.
%3) Low scalability because of unchangeable hardware


Our contributions are the following:
\begin{itemize}

\item A novel reconfigurable multi-threaded multi-core neural processing unit to enable effective and efficient multi-neural network execution for LSTM inferences. 

%\item A custom coarse-grained multithreading LSTM (CGMT-LSTM) hardware architecture is introduced which significantly improves the hardware utilization and also leads to significant performance improvement. 

\item A custom coarse-grained multi-threaded (CGMT) LSTM accelerator architecture that also can be partitioned into several full-fledged sub-accelerator cores, which significantly improves hardware utilization and design performance. 

\item A custom tiling method for LSTMs, which minimizes the intermediate results buffers when combining CGMT and partition, thereby increasing the accelerator area efficiency.

\item A comprehensive evaluation on the proposed methods and hardware architecture.

\end{itemize}

\subsubsection*{Relationship to Prior Publications:}
This article expands on a conference paper~\cite{que2020reconfigurable} with the baseline design proposed in~\cite{que2020optimizing}. The baseline design~\cite{que2020optimizing} involves a novel latency-hiding hardware architecture based on column-wise matrix-vector multiplication. It has much higher performance and hardware utilization than other designs for RNN models with different sizes, but it still suffers from underutilization when the model size is small. \cite{que2020reconfigurable} addresses the underutilization issue by introducing coarse grained multithreading (CGMT) which enables temporal multi-neural network execution to improve the performance when the RNN models are small while still maintaining the performance of RNN models with medium to large sizes. It mainly time-multiplexes a large RNN accelerator across various RNNs workloads. 
This article addresses a limitation of the work described in our previous papers, that they do not allow the large computation engine to be partitioned into several smaller ones, so they do not support spatial co-execution of multiple RNN inferences. This limitation brings a severe hardware underutilization issue when targeting acceleration for a large number of small RNN models which are commonly used in many applications~\cite{hundman2018detecting, que2021accelerating, zaremba2014recurrent, guan2017fpga}.
%The previous work~\cite{que2020reconfigurable} explores the multi-threading which mainly time-multiplexes a large RNN accelerator across various RNNs workloads. 
This work introduces an accelerator hardware architecture that can be partitioned into multiple full-fledged sub-accelerator cores, combining multithreading with multi-core techniques to enable temporal and spatial multi-neural network execution on cloud based NPUs. 
The proposed novel dimension of optimization allows us to obtain significant improvement in throughput while reducing latency over the previous design~\cite{que2020reconfigurable}.
This paper adds the design of multiple sub-accelerator cores for spatial co-execution of RNNs in~\secref{subsec:multicore}.  \secref{subsec:system}-\ref{subsec:system_others} describe a revised hardware architecture, and~\secref{subsec:to_gpu}-\ref{subsec:to_fpga} contain new evaluation results. 





%Relationship to Prior Publications: This article expands on a conference paper by Cheng et al.


%\newpage
\section{Background and Preliminaries}
%\subsection{Related Work}

%\subsection{LSTMs}
\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.8\linewidth]{img/lstm07.pdf}
\end{center}
   \caption{A diagram of an LSTM Cell.}
\label{fig:lstm}
\end{figure}


%LSTMs are artificial neural networks which have feedback connections and internal memory cells to record past information about long-term dependencies over an arbitrary time. They achieve high accuracy in many sequence processing problems such as text analysis, speech recognition and video classification. %Among the many RNN variants, the most two popular ones are LSTMs and Gated recurrent units (GRUs). 

RNNs/LSTMs have been shown to have useful properties with many significant applications. 
Among the many RNN variants, the most popular one is the LSTM which was initially proposed in 1997~\cite{hochreiter1997long}. 
This study follows the standard LSTM cell~\cite{guan2017fpga, fowers2018configurable, eriko_fccm19, lrcn_donahue2015long}.
\figref{fig:lstm} contains a diagram of an LSTM cell. 
It utilizes the following equations to compute the gates and produce the results for the next time step. 
%The hidden state $h_t$ is produced by the following equations:
%\begin{align*}
%    i_t &=\ \ \ \ \sigma(W_i[x_t, h_{t-1}] + b_i) \\
%    f_t &=\ \ \ \ \sigma(W_f[x_t, h_{t-1}] + b_f) \\
%    g_t &= tanh(W_g[x_t, h_{t-1}] + b_u)         \\
%    o_t &=\ \ \ \ \sigma(W_o[x_t, h_{t-1}] + b_o) \\
%    c_t &= f_t \odot c_{t-1} + i_t \odot g_t \\
%    h_t &= o_t \odot tanh(c_t)
%\end{align*}
\begin{align*}
%\vspace{-0.5cm}
    i_t &=\sigma(W_i[x_t, h_{t-1}] + b_i), 
    & f_t &=\sigma(W_f[x_t, h_{t-1}] + b_f) \\
    g_t &= \text{tanh}(W_g[x_t, h_{t-1}] + b_u), 
    & o_t &= \sigma(W_o[x_t, h_{t-1}] + b_o) \tag{1} \label{eq:1} \\
    c_t &= f_t \odot c_{t-1} + i_t \odot g_t, 
    & h_t &= o_t \odot tanh(c_t)
\end{align*}
Here, $\sigma$ and $tanh$ represent the sigmoid function and hyperbolic tangent function. Both are activation functions. $i_t, f_t, g_t$ and $o_t$ stand for the output of the input gate ($i$-gate), forget gate ($f$-gate), input modulation gate ($g$-gate) and output gate ($o$-gate) at timestep $t$ respectively. The $g$-gate is often considered as a sub-part of the $i$-gate. Each LSTM gate consists of a Matrix-Vector Multiplication (MVM) unit and a corresponding activation function unit, as shown in~\figref{fig:lstm}. 
The $\odot$ operator denotes an element-wise multiplication. $W$ is the weight matrix for both input and hidden units since the input vector and hidden vector are combined in the equations. The $b$ terms denote the bias vectors. $c_t$ is the internal memory cell status at timestep $t$ while $h_t$ is the hidden vector which is the output of the cell and passed to the next timestep calculation or next LSTM layer. 

The LSTM information flow is controlled by these four gates with details shown in~\figref{fig:lstm}. The $i$-gate decides what new information is to be written into the internal memory cell; the $g$-gate modulates the information processed by $i$-gate via adding non-linearity. Note that only $g$-gate utilizes hyperbolic tangent as its activation function while all the other three gates utilize sigmoid. The $f$-gate decides what old information is no longer needed and can be discarded so there are element-wise multiplications between the output of $f$-gate and memory cell status in the previous timestep $c_{t-1}$. Its output will be added to the products of the outputs from $i$-gate and $g$-gate to form the current status of the internal memory cell. 
The $o$-gate decides what the value of the current hidden vector ($h_t$) should be by multiplying the current status of the memory cell after the hyperbolic tangent function, as shown in the LSTM-Tail in ~\figref{fig:lstm}. 
Our work focuses on the optimization of RNN inferences involving  standard LSTMs, but the proposed techniques can be applied to other DNN inferences.


%\input{parameters.tex}


\section{Design and Optimization Methodology} \label{sec:design}
%In this section, the overview of the proposed design is first presented. Then several software and hardware optimization techniques are proposed. 
%Since most of the calculations of LSTM cells lie in the MVM with complex data dependencies, this paper will focus on optimizing the MVM of LSTM for high throughput. The other operations, like the element-wise operations in the LSTM tail, can work under the shadow of the MVMs. 

Accelerating RNN/LSTM inferences efficiently is challenging because of their recurrent nature and data dependencies. This section first presents the coarse-grained multithreading for accelerating RNN/LSTM and then introduces a partitioning strategy of LSTM weight matrix to apply sub-layer granularity scheduling with fine-grained tasks for Remarn architecture. Finally, we present the multi-core accelerator to enable spatial co-execution of RNN models or layers to improve the design performance.
%This section introduces the proposed optimization in detail. 
Some design parameters are defined in Table \ref{tab:BBP}. 
%We define a few parameters, as shown in Table \ref{tab:BBP} for later calculations.
\input{param.tex}

\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.8\linewidth]{img/multi_task_cgmt_t01.pdf}
\end{center}
   \caption{Timeline of three LSTM tasks based on the proposed coarse grained multithreading.}
   \vspace{0.2cm}
\label{fig:cgmt}
\end{figure}

\subsection{Multithreading for Recurrent Neural Processing Unit}\label{subsec:Multithreading}

There is a large demand for architectural support of multi-DNN execution to maximize the hardware utilization and reduce the costs of running a large-scale production system. However, most of the existing LSTM accelerators can only run one task at a time~\cite{mittal2021survey, fowers2018configurable, eriko_fccm19, que2020optimizing, han2017ese,guan2017fpga}. This work proposes a coarse-grained multi-threaded (CGMT) LSTM NPU which switches on the event when the data hazard of a computational unit happens in the LSTM computation. 
The general idea is when a thread is stalled because of some events, e.g., cache misses, the multi-threaded core can switch to a different hardware context. In the proposed CGMT LSTM accelerator, the event is the hazard caused by the data dependency between the timesteps of sequential calculation in LSTMs. 
We propose to maintain multiple thread contexts in a recurrent NPU core so that when the first thread stalls, the second one can carry on, as shown in~\figref{fig:cgmt}. Thus, it utilizes computational resources more efficiently than a single thread core. It can increase the design performance by utilizing thread-level parallelism and enhance the NPU hardware utilization. 
%It also helps to reduce context switch penalty. 

Besides, a preceding LSTM model or layer may have thousands of sequences (timesteps), which occupies the NPU core for a long time, leading to a long waiting time for the latter requests before they have an available core to run. However, some services have strict latency constraints since the response time directly relates to user experience, e.g., intelligent personal assistants are one of the examples where real-time DL is utilized to handle user speech and output smart responses. The conventional single-threaded NPUs can only store the old thread's context to memory and retrieve the new thread's context using preemption mechanisms~\cite{choi2020prema} to run another task. However, it will have a large context switch penalty. In our multi-threaded NPU for LSTMs, the new task can execute from another thread as soon as it comes, as shown in~\figref{fig:cgmt}. Please note that a particular thread may still stall due to data hazard, but the physical core is not stalled since multiple threads share the same computational physical core, which leads to "Virtual idle" as shown in this figure. 
We believe that further optimizations, e.g., simultaneous multithreading (SMT) can be adopted to our NPU design to gain even higher performance. We leave it for our future work because it does not have a big impact on the conclusions we draw from this work. 

%Traditionally, the processor keeps track of the context of a single thread. 
%When it is doing multiple tasks and a new thread needs to be executed, old thread’s context in hardware written back to memory and new thread’s context loaded. 


%They note that in an LSTM, the sequence length greatly exceeds the number of layers. For example, a 4-layer LSTM may process a sequence of length above 20. Based on this, they propose a scheduling scheme, where the computation tasks of every timestep are grouped into multiple threads. Mapping 27 of threads to cores is done in interleaved fashion and then, scheduling is done while respecting datadependencies.

%\subsection{Fairness in Coarse-grained Multithreading}
%Resource sharing in space and time always causes fairness
%considerations. 



\subsection{Weights Matrix blocking Strategy}\label{subsec:blocking}

The LSTM calculation of one timestep in an LSTM layer has 4 MVM operations according to the equations~\eqref{eq:1}. Besides, these four MVM are independent and share the same size. Since the 4 matrices of $i, f, o, u$ gates in LSTMs have the same size, these matrices can be combined into a single large matrix~\cite{abdelfattah2018dla, que2020optimizing}. \figref{fig:matrix} illustrates the basic idea. 
Thus, in the calculation of one timestep of an LSTM layer, we can only focus on the optimizations of one large matrix multiplying one vector for the whole LSTM cell rather than 4 small matrices multiplied by one vector. This is a general optimization that can be utilized for any MVM operations which share the same input vector. Because each matrix from LSTM gates has a size of $Lh \times (Lx+Lh)$, the large fused matrix has a size of $(4 \times Lh) \times (Lx+Lh)$.

%With the combined matrix, each of the LSTM gates are computed one-after-the-other since we compute the matrix


%To describe our scheduling granularity, we define sub-layer as a single PE array mapping (i.e., single iteration). 

%\begin{figure}%[ht]
%\begin{center}
%\includegraphics[width=0.5\linewidth]{img/blocking03.png}
%\end{center}
%   \caption{The combined weights matrix, showing the sub-layers. The number of sub-layers are 4 in this example.}
%\label{fig:blocking}
%\end{figure}



Usually, deep neural networks have many compute intensive operations involving large weight matrices, which can be accelerated by running in parallel. 
However, when deploying on FPGAs, the parallelism is constrained by the limited hardware resources on the targeted FPGAs. It means that the whole MVM computation may not be fully unrolled and performed at once, especially for the large LSTMs. 
To use the computational resources efficiently, the combined weight matrix of an LSTM layer is partitioned into multiple sub-layers in advance depending on the configuration of the accelerator cores and LSTM layer sizes. 
%As the accelerator configuration determines the size of a sub-layer, 
Specifically, an LSTM layer of one timestep is partitioned into a number of sub-layers with equal size, as shown in~\figref{fig:blockinga}. For simplicity, the number of the sub-layers in the example is set as 2 to illustrate the idea, but a real design could have more sub-layers and it depends on the design constraints. 
And then, Element-based Parallelism (EP) and Vector-based Parallelism (VP) are applied to exploit the available parallelism~\cite{que2020optimizing}. The number of the sub-layers is determined by $\frac{(4 \times Lh)}{VP}$. 
The sub-layer is then divided into many small tiles, each having a size of $(EP, VP)$, as shown in~\figref{fig:blockingb}. In each cycle, our Remarn core is able to process the MVM of a tile and a sub-vector of $[x_t, h_{t-1}]$ with a size of $EP$. 
%$EP$ and $VP$ need to be carefully determined so that the number of cycles to process the $x_t$ vector, given by $\frac{Lx}{EP}$, is larger than the system latency to make sure the computation of hidden vectors can be hidden by processing $x_t$ vector. This number is small when $EP$ is large and it may still result in system stalls. 
To increase the design parallelism, $VP$ should be chosen to be as large as possible. However, the largest value of $VP$ equals $Hw$, which is $4 \times Lh$, since there are only four gates in an LSTM. Thus, the smallest number of sub-layers is one when $VP$ is $4 \times Lh$. In this study, sub-layer granularity scheduling is adopted with fine-grain tasks of sub-layers for multi-LSTM execution.
Besides, we interleave the rows of the four weight matrices, so that the related elements from the four gates output are adjacent in the result vector. Thus, the LSTM gate outputs can multiply with each other easily using the element-wise operations in the LSTM-tail unit. It also means that there is no data dependency between these sub-layers. 
%When the proposed CGM-LSTM core switch to another thread, 
The optimization of interleaving also removes the requirement to buffer large intermediate outputs from 4 LSTM gates since the result sub-vectors from the sub-layers are not related and will be reduced in the tail unit soon. Each sub-vector of the MVM output can be handled individually in the LSTM-tail units. There is no need to wait for other sub-layer results to get the LSTM memory cell status and hidden vector of the current sub-layer. 
%It may be both natural and right when blocking CNNs since CNNs are forward 
The proposed CGMT core will always finish processing all the sub-layers in one timestep before it switches to another thread because the data hazard in the LSTMs happens when timestep changes. 
Compared with a fine-grained multithreading scheme which switches the context between threads in every cycle, we can avoid buffering these large intermediate MVM operation values as well as element-wise operation values since these values will finally form the sub-vectors of LSTM memory cells and hidden units. 
Only the thread dedicated buffers are needed to be added for storing the LSTM memory cells and hidden units in each timestep since different threads process different LSTM tasks. 

\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.8\linewidth]{img/matrix_fusion_t01.pdf}
\end{center}
   \caption{The four weight matrices from the four LSTM gates and the fused weight matrix. The weights from the four gates are interleaved. The lengths of the input vector and hidden vector are 2 in this figure.}
  % \vspace{0.2cm}
\label{fig:matrix}
\end{figure}



\begin{figure} 
   \centering
  \hspace*{\fill}
  %\centering
  \subfloat[\label{fig:blockinga}]{%
    \includegraphics[width=0.30\linewidth]{img/blocking_t01.pdf}}
  \hfill
  %\centering
  \subfloat[\label{fig:blockingb}]{%
    \includegraphics[width=0.42\linewidth]{img/sublayers_t01.pdf}} \hspace*{\fill}

  %\hspace*{\fill}
  %\vspace{ 0.3 cm}
  \caption{The partition of an LSTM weight matrix. (a) The fused weight matrix, showing two sub-layers. (b) The MVM of a sub-layer based on a tile of $EP \times VP$ shaded in blue.}
  \vspace{ 0.2 cm}
  \label{fig:blocking} 
\end{figure}


%With a fine-grained multi-threading scheme, we may still need to buffer these intermediate gate values since we


%Furthermore, since the sub-layers are scheduled to process in sequences, the sub-vector of LSTM memory cell can also be stored in each LSTM-tail units  

%as each of the input/forget/output gate values will now need to be buffered (using costly on-chip RAM or slow external memory) so that they can be combined in the second half of the LSTM cell

%This removes the need for buffering large intermediate gate outputs, and allows us to directly stream the gate values into the dedicated LSTM hardware block. 
\iffalse
\begin{figure} 
   \centering
  \hspace*{\fill}
  %\centering
  \subfloat[\label{fig:layers}]{%
    \includegraphics[width=0.50\linewidth]{img/layer_t02.pdf}}
  \hfill
  %\centering
  \subfloat[\label{fig:layer_pipeline}]{%
    \includegraphics[width=0.42\linewidth]{img/layer_pipeline_t02.pdf}} \hspace*{\fill}

  %\hspace*{\fill}
  %\vspace{ 0.3 cm}
  \caption{Intra-model parallelism of a LSTM model. (a) A multi-layer LSTM model showing intra-model data dependencies after unfolding. The number of layers and timesteps is three and four in this example. $c_{ij}$ represents the cell state of layer $i$ and timestep $j$. (b) Layer and timestep overlapping showing the Parallelism using three sub-accelerator cores.}
  \vspace{ 0.2 cm}
  \label{fig:lstm_layers} 
\end{figure}
\fi





\subsection{Multi-core for Recurrent Neural Processing Unit}\label{subsec:multicore}
Many RNN/LSTM accelerators deploy all the computing resources to form a single accelerator core with a large scale, leveraging data-level parallelism. However, this type of accelerator is only able to process one task at a time, resulting in potential underutilization and inefficiency when multiple tasks come at the same time, especially in large data centers. Multithreading described in~\secref{subsec:Multithreading} can address the issue partially but it is still suffering to deal with a large number of small workloads. Recently, spatial architectures have become a popular solution to build high throughput accelerators for deep neural networks (DNNs)~\cite{venieris2018f,ghodrati2020planaria, wang2021metro}. Generally, multiple PEs are grouped as an engine and these engines are connected with an on-chip interconnection to enable data communication during processing.
f-CNN$^x$~\cite{venieris2018f} proposes multiple custom dedicated engines for the workloads with various CNN models. Planaria~\cite{ghodrati2020planaria} proposes to dynamically fission a systolic array based DNN accelerator at runtime to spatially co-locate multiple DNN inferences. However, none of them targets RNNs, and they do not consider the recurrent nature and data dependency in RNN computations which are absent from accelerators targeting CNNs and fully connected (FC) layers. 
%This work adopts the similar idea to~\cite{ghodrati2020planaria} but targets a Brainwave style~\cite{fowers2018configurable, eriko_fccm19, que2020optimizing} accelerator for accelerating RNNs. 
This work adopts a similar idea to~\cite{ghodrati2020planaria}. But instead of using a systolic 2-dimensional matrix-matrix multiplication array, our architecture uses matrix-vector multiplication engines since RNNs and MLPs are dominated by matrix-vector multiplication operations. 
With multiple sub-accelerator cores, it enables spatial co-execution of multiple RNN/LSTM inferences on the same hardware and offers simultaneous multi-RNN accelerations. 


\begin{figure}%[ht]
\begin{center}
\includegraphics[width=1.0\linewidth]{img/layer_pipe_design_t09.pdf}
\end{center}
   \caption{ Two LSTMs (A and B) are mapped to Remarn. 
   (a) A multi-layer LSTM model showing intra-model data dependencies after unfolding. The number of layers is three and the number of timesteps is four in this example. Layer 0/1/2 are labeled in green/yellow/blue respectively. $c_{ij}$ represents the cell state of layer $i$ and timestep $j$.
   (b) Computation order for minimum data dependencies. 
   (c) Two LSTMs are mapped to a single-thread single-core design.
   (d) Two LSTMs are mapped to a three-thread single-core design.
   (e) Two LSTMs are mapped to a single-thread three-core design.
   (f) Two LSTMs are mapped to a dual-thread three-core design.
   }
   \vspace{0.2cm}
\label{fig:lstm_layers}
\end{figure}



In addition to inter-model parallelism which is naturally supported by using multiple sub-accelerator cores, such as co-execution of multiple models, our design also enables intra-model parallelism among different layers and timesteps of the RNN layers. Generally, in an RNN model, a latter layer or timestep should wait until its preceding layer or timestep finishes since some of its inputs are the output of the preceding layer or timestep, as shown in~\figref{fig:lstm_layers}(a). E.g., the computation that requires $c_{00}$ and $h_{00}$ cannot start until they are available from the preceding layer or timestep. 
Using a single-threaded single-core accelerator, two LSTM workloads will run as ~\figref{fig:lstm_layers}(c) shows. The accelerator will process the LSTM layers and timesteps iteratively. The temporal inefficiency comes from the stall of data dependencies and the spatial inefficiency comes from a small network mapping to a large core leaving some resources idle. 
With a multi-threaded accelerator, each layer of the LSTM can run on different threads to remove the stall or the temporal inefficiency which comes from the RNN nature data dependencies. Please note, a special computation order, as shown in~\figref{fig:lstm_layers}(b) is required to achieve stall-free processing using a multi-threaded single-core accelerators, as shown in~\figref{fig:lstm_layers}(d).
However, when LSTMs are small, many resources are left unused when mapping them to a large core. In such cases, a small core will get a similar latency to the one using a large core. Besides, with multiple sub-accelerator cores, the processing of the cascaded LSTM layers can be overlapped in a layer-wise coarse-grained pipelining as shown in~\figref{fig:lstm_layers}(e). The second layer does not need to wait for the whole sequence of hidden vectors of the first layer to be ready. Just one hidden vector from the preceding LSTM layer is sufficient to start the calculation of the next LSTM layer. It helps to reduce the overall design latency. Besides, since the output of the preceding layer sinks directly in the following sub-accelerator core, there is no need for buffering large intermediate outputs, which could help to improve the area efficiency. 
We can further optimize the processing after combining the multithreading with multi-core. \figref{fig:lstm_layers}(f) shows two LSTMs are mapping to a dual-thread three-core accelerator, which achieves the best total latency. 

While the multi-core scheme leads to high performance, it also presents a new challenge: in some situations it can not provide sufficient bus bandwidth per core. In Remarn, the multiple cores share the same front side bus. But this will not affect on the bus bandwidth because we do not add new Remarn big cores but only split the original big core into several small ones, e.g., four small cores. When the four small cores co-operate to handle a large network, the quad-core requires the same bandwidth as the one with a big monolithic core. The total bus bandwidth they require is the same as the large core from which they are derived, which is smaller than that for 4 large cores. 
%When the four small cores operate concurrently on different smaller networks, the total input is small. With multiple small networks, the bandwidth requirement of the design is lower than the one with a big network. 
%For example, the size of four small LSTM models with $L_h=64$ is much lower than the size of one big LSTM model with $L_h = 1024$. 
For example, the bandwidth requirement of four small LSTM models with $L_h=64$ is much lower than the one of one big LSTM model with $L_h=1024$. 




%Combining the time-multiplexing introduced in~\secref{subsec:Multithreading}, our design can provide more parallelism 

%Besides, temporal multi-tenancy is combined to enable a further exploration of the parallelism. Our design which can be split into multiple sub-accelerators targeting a brainwave-like architecture


%~\cite{kwon2021heterogeneous} propose heterogeneous dataflow accelerators, which are composed of multiple sub-accelerators with different hardware architectures of dataflow, to support spatial co-execution of multi-tenant workloads.


%It involves six matrix-vector multiplication (MVM) ``tile engines", each processing $400\times 40$ matrices. The results of the tile engine are fed to a balanced adder-tree, so these engines can effectively process a $400\times 240$ matrix in parallel. Any MVM that does not map to this dimension will leave some resources idle.

\iffalse

\subsection{Scheduling}\label{subsec:schedule}

\newpage 
\subsection{Scheduling and Optimizations}

\textcolor{red}{Notes: This subsection is about \textcolor{blue}{Dynamic Scheduling and Static Scheduling}. This note only used for showing the topic of this subsection and will be deleted later.}

The scheduling strategy for multi-core accelerators for DNN workloads is a new and rarely explored topic. PREMA~\cite{choi2020prema} introduces a preemptive scheduling algorithm on a single-core NPU to support multi-DNN execution. AI-MultiTasking~\cite{baek2020multi} proposes to process different neural networks by partitioning their various layers into identical sub-layers in compile time. It also develops a heuristic of mapping DNN jobs to the accelerator. 
%It exploits three scheduling mechanisms, including First-In-First-out (FIFO), Round-Robin (RR), and greedy algorithm. The RR scheduling repeatedly selects one sub-layer from different neural networks. 
In~\cite{kwon2021heterogeneous} Heterogeneous Dataflow accelerators (HDAs) are proposed to support the heterogeneous acceleration of multi-DNN workloads using manual-designed mapping of jobs to sub-accelerators and compile time layer scheduling. 

We exploit the intra-model data-dependencies of both timesteps and layers in LSTMs, as shown in~\figref{fig:lstm_layers}(a). Both the dependencies have a linear dependence chain in the model. For LSTM inferences, it is processed from the first layer to the last layer sequentially and from first timestep to the last timestep in each layer. Besides, layers from different LSTMs are independent. This work develops a set of heuristics which exploit the characteristics of LSTM inference workloads to reduce the overhead of the scheduling for the proposed multi-core accelerator. 
A runtime scheduler is maintained on the host side. Once the scheduler knows the parameters (e.g. the timesteps, the number of layers) of an LSTM, it knows the structure of the model and so the processing time is predictable.
It partitions all the coming LSTM requests into layer-wise jobs and distributes the first unscheduled layers from various requests into $N$ ($N=4$ in this work) core-dedicated queues, each for a sub-accelerator core, with the ordering of First-Come-First-Served (FCFS) and load balancing. Each sub-accelerator core accesses the dedicated queue and execute the LSTM layers by interleaving timestep executions in LSTM layers with multiple threads. Different dynamic scheduling strategies are possible, but evaluating which one would produce the best results under which conditions is challenging and would be addressed in future research. 

The accelerator can also be customized using static scheduling which does not have the complexity and run-time overheads of dynamic scheduling. 
With manual-designed scheduling, a fine-grained scheduling strategy can be applied, which partitions a large layer into several sub-layers as shown in~\secref{subsec:blocking} and then schedules these sub-layers together as long as there are sufficient sub-accelerator cores. It enables multiple sub-accelerator cores to work together to execute a large layer. 
The manual and static scheduling examples illustrate the best case situations, which show the upper bound of what can be achieved statically and show what the best case situations look like. In future, we will support the fine-grained scheduling dynamically, such as using Gang scheduling which schedules a gang of jobs onto free cores. Besides, more other sophisticated scheduling strategies will be added, tested and compared. 

%if all the LSTM requests have the same hidden size, e.g., when running only one application. A fine-grained static scheduling can be applied, which partitions a layer into several sub-layers as shown in~\secref{subsec:blocking} and then schedules these sub-layers together as long as there are sufficient sub-accelerator cores. It enables multiple sub-accelerator cores to work together to execute a large layer. In future, we will support the fine-grained scheduling dynamically in our accelerator, such as using Gang scheduling which schedules a gang of jobs onto free cores. Besides, more other sophisticated scheduling strategies will be added and tested.
%~cite{ousterhout1982scheduling}

%A global candidate queue is maintained on the host side with all the coming requests. It includes all the first unscheduled layers from various coming LSTM requests, which can be scheduled immediately without waiting for other data. 


\subsection{Scheduling and Optimizations}\label{subsec:schedule}

\textcolor{red}{Notes: This subsection is about \textcolor{blue}{Pure Static Scheduling}. This note only used for showing the topic of this subsection and will be deleted later.}

%\textcolor{blue}{

The scheduling strategy for multi-core accelerators for DNN workloads is a new and rarely explored topic. PREMA~\cite{choi2020prema} introduces a preemptive scheduling algorithm on a single-core NPU to support multi-DNN execution. AI-MultiTasking~\cite{baek2020multi} proposes to process different neural networks by partitioning their various layers into identical sub-layers in compile time. It also develops a heuristic of mapping DNN jobs to the accelerator. 
%It exploits three scheduling mechanisms, including First-In-First-out (FIFO), Round-Robin (RR), and greedy algorithm. The RR scheduling repeatedly selects one sub-layer from different neural networks. 
In~\cite{kwon2021heterogeneous} Heterogeneous Dataflow accelerators (HDAs) are proposed to support the heterogeneous acceleration of multi-DNN workloads using manual-designed mapping of jobs to sub-accelerators and compile time layer scheduling. 
Inspired by~\cite{baek2020multi, kwon2021heterogeneous} which rely on manually-designed heuristics, this work develops a set of heuristics which exploit the characteristics of LSTM inference workloads to reduce the overhead of the scheduling for the proposed homogeneous multi-core accelerator. 

We exploit the intra-model data-dependencies of both timesteps and layers in LSTMs, as shown in~\figref{fig:lstm_layers}(a). Both the dependencies have a linear dependence chain in the model. For LSTM inference, it is processed from the first layer to the last layer sequentially and from first timestep to the last timestep in each layer. Besides, layers from different LSTMs are independent. Once the scheduler knows the parameters (e.g. the timesteps, the number of layers) of an LSTM, it knows the structure of the model and so the processing time is predictable. 
This work adopts static scheduling, which does not have the complexity and run-time overheads of dynamic scheduling. It shows the upper bound of what can be achieved statically and shows what the best case situations look like. 
Based on the characteristics of LSTM inference workloads, this work schedules the workload in a layer order and in a timestep order when in a layer.
Besides, each LSTM layer is partitioned into several sub-layers as shown in~\secref{subsec:blocking}. A group of sub-layers are then scheduled together with each sub-layer running on a sub-accelerator core. It enables multiple sub-accelerator cores to work together to execute a large layer. 
In future, we will support the fine-grained scheduling dynamically in our accelerator, such as using Gang scheduling which schedules a gang of jobs onto free cores. Besides, more other sophisticated scheduling strategies will be added and tested.
%}


%Besides, this work also interleaves the execution of timesteps of layers from different LSTMs. Our scheduler implements a greedy method with latency as the metric. We extended the cycle-accurate simulator in~\cite{que2020optimizing} to support the multiple sub-accelerator cores environment to estimate the layer latency. However, if there are large unbalanced loads across cores, e.g., one core has a much larger latency than others, our scheduler explores alternative scheduling and tries to reduce overall latency. In future work, more sophisticated scheduling strategies will be added and tested. }


%\textcolor{blue}{The scheduling strategy for multi-core accelerators for DNN workloads is a new and rarely explored topic. Inspired by~\cite{baek2020multi, kwon2021heterogeneous} which rely on manually-designed heuristics, this work develops a set of heuristics which exploit the characteristics of RNN inference workloads to reduce the overhead of the scheduling for the proposed homogeneous multi-core accelerator. We exploit the intra-model data-dependencies of both timesteps and layers in RNNs, as shown in~\figref{fig:lstm_layers}(a). Both the dependencies have a linear dependence chain in the model. For RNN inference, it is processed from the first layer to the last layer sequentially and from first timestep to the last timestep in each layer. Besides, layers from different RNNs are independent. Based on these characteristics of RNN inference workloads, this work schedules the workload in a layer order and in a timestep order when in a layer. Besides, this work also interleaves the execution of timesteps of layers from different RNNs. }

%\textcolor{blue}{Our scheduler implements a greedy method with latency as the metric. Although RNNs can receive any variable length input sequence, the length of the input timestep (sequence) is fixed in inference~\cite{choi2020prema}. Predicting the temporal unrolled recurrence length for RNN workloads is negligible as it is statically determined by the input sequence length. We extended the cycle-accurate simulator in~\cite{que2020optimizing} to support multiple sub-accelerator cores environment to estimate the layer latency. However, if there are large unbalanced loads across cores, e.g., one core has a much larger latency than others, our scheduler explores alternative scheduling to reduce overall latency. Currently we do not exploit a dynamic scheduling strategy since it comes at the cost of run-time overhead that can affect parallel execution efficiency. In future work, more sophisticated scheduling strategies will be added and tested. }


\newpage

\fi

\section{Hardware Architecture}
Based on the optimization techniques introduced above, we implement the proposed Remarn on top of a state-of-the-art (SOTA) RNN accelerator~\cite{que2020optimizing} for low latency cloud-based applications. In~\secref{subsec:big-little}, we outline the main components of the architecture and detail the necessary hardware modifications required in order to support our Remarn unit. 
%Several FPGA-specific optimizations along with data quantization are also introduced.
Several FPGA-specific optimizations are also introduced. 



\subsection{System Overview}\label{subsec:system}
A high-level block diagram of Remarn accelerator is shown in~\figref{fig:system}(a) and~~\figref{fig:system}(b). The original monolithic accelerator with all the MVM kernels in our previous work~\cite{que2020reconfigurable} has been split into $N$ (e.g., $N=4$ in the figure) sub-accelerator cores, each working in a big-little engines architecture. All these $N$ cores are connected via the switch for hidden vectors and partial sum data movement. When $N$ is small as in this case, the switch can be implemented by a crossbar. When $N$ is large, then a network-on-chip could be more effective. 
%It would be our future work to find out how the implementation of the switch and the whole accelerator varies with $N$. 
Hence, in one extreme, all the 4 cores can be attached together to construct a large logical accelerator, running only one RNN inference using the entire accelerator. Alternatively, it can also provide 4 standalone sub-accelerator cores, spatially co-executing 4 different RNNs simultaneously. Combining with the CGMT of 4 threads, it can support up to 16 different RNN inferences simultaneously. 
In this work, all the sub-accelerator cores are identical. But the design can be extended easily to employ a different accelerator hardware architecture, e.g., a systolic array-based one, for some of the cores to support the heterogeneous acceleration of multi-DNN workloads~\cite{kwon2021heterogeneous}.
This work utilizes a general switch as the interconnection between the cores, which brings a slight performance drop when fusing as a large accelerator compared to a monolithic one since the computational engines now need one more hop to share the partial results. 
%More recently, the METRO~\cite{wang2021metro} is proposed to alleviate the inefficiency of the interconnection for Spatial DNN accelerators. 
We leave that for future work since it has a limited impact on the conclusions we draw from our study in this paper.

\begin{figure}%[ht]
\begin{center}
\includegraphics[width=1.0\linewidth]{img/design_overview_t06.pdf}
\end{center}
   \caption{Overview of the design.}
   \vspace{0.2cm}
\label{fig:system}
\end{figure}


%\vspace{-0.2cm}
\subsection{The Big-Little Engines Architecture}\label{subsec:big-little}
This work proposes a hardware architecture with big-little engines for the DNN accelerators, which is illustrated in~\figref{fig:system}(a). 
The proposed accelerator core consists of a big engine, a little engine, an adapter unit, the crossbar as well as weight and vector buffers. The big engine is for the matrix operations which are computation intensive while the little one is for the small but essential components in the neural networks, such as ReLU, pooling, batch normalization, activation etc. The big-little engines architecture follows a wait-free single-producer/single-consumer mechanism using the adapter unit, which adjusts the data parallelism between the two engines.  
In this work, the big engine unit has $VP$ MVM kernels to perform matrix-vector multiplications for LSTM gates operations. It occupies the major computational resources, such as DSPs. 
Practically, the design will deploy a large number of hardware resources in the big engine to increase the data parallelism to improve the processing ability. However, since the big engine produces one output vector after multiple accumulation cycles, 
the little engine does not require a large parallelization factor by deploying many LSTM tail units like the one in the big engine unit. 
The adapter unit can convert the parallelism between the two engines. With a proper adapting factor between the big engine output and little engine input, the little engine can be fully occupied without a stall or wait. The little engine unit has a vector activation function unit and $EP$ tail units which execute the element-wise operations in the LSTM computation. It does not contain many computation resources like the big engine, but it is essential for running the whole neural networks on-chip. 

Besides, with different hardware components in the little engine, such as ReLU, pooling, batch normalization etc, our design can easily be extended to support other types of neural networks, such as CNNs. The Brainwave~\cite{fowers2018configurable} accelerate and serve CNN models using its MVM engines and custom multi-function units. Sometimes, to accelerate DNN designs, the big engine can be a large systolic array supporting large matrix operations and the little engine utilizes a SIMD vector unit to support general vector operations~\cite{ghodrati2020planaria} for the other operations in NNs.
The LSTMs are much more challenging to accelerate, exhibiting lower available parallelism and more data dependencies than 2D CNNs~\cite{fowers2018configurable}.
This design focuses on accelerating RNN/LSTM inferences using a brainwave-like architecture, but the proposed optimizations and hardware architecture can be easily extended to support other neural networks, which will be our future work. 


\vspace{0.3cm}
\subsection{Detailed Hardware Components in one sub-accelerator core}\label{subsec:system_others}
\subsubsection{Overview of the sub-accelerator core}
Each sub-accelerator core is a full-fledged RNN neural processing unit with coarse-grained multithreading. It has many logical NPUs that share nearly all resources of the physical NPU, e.g., weights buffer, kernel units, activation function units, element-wise units, as shown in~\figref{fig:system}(a). 
%In the next subsections, we outline the main components of the architecture and detail the necessary hardware modifications required in order to support our CGM-LSTM scheme.
The core has $VP$ MVM kernels, each having $EP$ Processing Elements (PEs), resulting in $VP\times EP$ available PEs. 
The $VP$ and $EP$ values are determined via the design space exploration described in~\cite{que2020optimizing}. In this paper, each PE is one fully pipelined multiplier. The kernels are used to perform the matrix-vector multiplications between the weights and ${x_t}$ as well as ${h_{t-1}}$ that is required in LSTM gates operations shown in equations~\eqref{eq:1}. 

\subsubsection{The MVM Kernel Units}
Generally, the row-wise MVM is based on an architecture with parallel multipliers followed by a balanced adder tree. Accumulating the products of these multiplications is usually achieved using a balanced adder tree structure so that a number of related additions can be scheduled in parallel, which minimizes the overall latency of the system.
This architecture of the kernel unit is commonplace in FPGA-based designs of RNNs~\cite{guan2017fp,rybalkin2017hardware}. 
Since the elements in the partial result vector are not related, we adopt the column-wise MVM~\cite{que2020optimizing} that is based on the architecture of parallel multipliers followed by parallel accumulators. Besides, to support element-based parallelism, a small balanced adder tree is placed between the multipliers and the accumulators as shown in \figref{fig:system}{c}. This adder tree can help to balance $EP$ and $VP$ to improve parallelism.

In our proposed multi-threaded NPU core, all the logical cores share all the MVM kernel units. When one logical core (thread) is stalled, the other can still conduct calculations using the same kernel units. Thus, the proposed CGMT NPU core can utilize the resources of MVM kernels efficiently to improve the NPU performance and hardware utilization. Since each thread requires its own input vector $x_t$ and $h_{t-1}$, the design has to maintain multiple contexts by using buffers in the thread-aware vector manager and buffers unit. The thread selection logic is necessary to choose the required buffer to retrieve the data and conduct the remaining computations.

%\begin{figure}%[ht]
%\begin{center}
%\includegraphics[width=0.6\linewidth]{img/lstm_tail03.png}
%\end{center}
%   \caption{The LSTM-tail unit}
%   \vspace{0.2cm}
%\label{fig:tail}
%\end{figure}

%\subsubsection{The De-Quant unit}
%De-quantization (De-Quant) is applied to convert quantized values into fixed-point values to reduce hardware resources. Unlike the kernel units which mainly contain dot product operations, each of the tail units is composed of a sequence of element-wise operations, which can introduce frequent de-quantization and quantization operations in the linear-quantization scheme. Since de-quantization and quantization require a 32-bit multiplier unit and an adder, the total hardware cost of linear-quantization for the tail unit is higher than that of 16-bit fixed-point quantization. Therefore, we do not perform linear-quantization in the tail units. Instead, the quantized values will be de-quantized into fixed-point values. 

\subsubsection{The activation function unit}
The $\sigma~/~tanh$ unit performs the vector-based sigmoid ($\sigma$) and hyperbolic tangent ($tanh$) operations. They are implemented using programmable lookup tables with size of 2048 similar to~\cite{han2017ese, eriko_fccm19}. 
The implementation using lookup tables brings several benefits. First, our NPU can run a trained model with custom activation functions (e.g., a hard sigmoid from Keras~\cite{chollet2015keras}) from our users without re-training of the model. Because the equations of the custom sigmoid/tanh are not changed in the model, re-training is unnecessary. More importantly, we do not touch the sensitive data of users, which is vital for many users. Second, the lookup table has a fixed latency (e.g., 1 cycle) but other implementations, e.g., a piece-wise linear approximation, may involve multiplications that have a much larger pipe stage and latency. 

\subsubsection{The LSTM tail units}
\figref{fig:system}{d} illustrates the LSTM-tail units which perform the element-wise operations in the equations~\eqref{eq:1}. The LSTM memory cell FIFOs are employed to temporarily store the status of the running LSTMs since one thread may be switched due to data hazard before the design finish the calculation of the current LSTM layer with multiple timesteps. Because these threads are performing different LSTM layers or models, the design must keep multiple contexts of cell status of LSTMs, as shown in~\figref{fig:system}{d}. Other hardware contexts, such as the input data and hidden units, are maintained in the thread-aware vector manager and buffer unit with the same mechanism. 

%The output hidden vector ($h_t$) needs the quantization (Quant) before it can be used in the MVM kernels, so a Quant unit is utilized after the final output of LSTM-tail units as shown in \figref{fig:system}. 

%to reduce hardware resources since the Tail unit is composed of a sequence of element-wise operations, which can introduce frequent de-quantization and quantization operations using our quantization scheme.
%The Sigmoid ($\sigma$) and hyperbolic tangent ($tanh$) functions are implemented using lookup tables of size 2048 \cite{han2017ese, eriko_fccm19}. The LSTM-tail unit as shown in \figref{fig:tail} and GRU-tail unit mainly perform the element-wise operations. Several FIFOs in these tail units are utilized to synchronize the data and they are not shown in the figure. The output hidden vector ($h_t$) needs the quantization (Quant) before it can be used in the MVM kernels, so a Quant unit is utilized after the final output of LSTM-tail units as shown in \figref{fig:system}. 





%The proposed hardware architecture for neural network implementation is presented in this section.




\subsection{FPGA-Specific optimizations} \label{subsec:HyperFlex}
Since the proposed accelerator core can process a small tile with a size of $(EP,VP)$ in each cycle, all the MVM kernel units in one core share the same input of a sub-vector of $(x_t, h_{t-1})$, which has $EP$ elements. These $EP$ elements are broadcasted to all the MVM kernels for the computation. In addition, the design also needs to broadcast a single address to all the weight buffers units to fetch the weights. 
To alleviate the issue of large fan-out, the tree-shaped~\cite{eriko_fccm19} inter-connection is adopted to decrease the fan-out of each node with pipeline stages between the source and destination. The RTL code is carefully written to enable the use of HyperFlex registers on Stratix 10 to get high operating frequency~\cite{tan2018evaluating, Intel_hyperflex_wp}.

%We carefully wrote our RTL to enable the use of Stratix 10 HyperFlex registers to achieve higher operating frequency.

%We also implement a star-shaped interconnect for the paths from the central MVU logic to multiple MVU tiles and from the last MFU to multiple VRFs across the NPU, such that a distinct pipelined path is dedicated for each destination.

The DSP blocks in modern FPGAs, which are highly configurable, are often underutilized when implementing 8-bit DNN systems. \cite{xilinx_8bit} illustrates methods to extract two INT8 multipliers from Xilinx DSP48E2 Blocks which contain a 27x18 multiplier. \cite{intel_8bit} introduces a method to pack 2 INT8 multiplications into one INT18 multiplier with extra ALMs. Both the methods require two multiplications to share one input operand. In the column-wise architecture~\cite{que2020optimizing}, the computation order of MVM is different from the one in row-wise MVM. With the column-wise MVM used in RNN designs, one column of the weights matrix naturally shares the same element of the input vector and conducts the multiplications at the same time. Thus, these multiplications share one input operand, which helps us to pack four INT8 multiplications into one DSP block on Intel FPGAs \cite{intel_8bit} to decrease the hardware resources. In addition, this would not be a restriction (and will come at a lower cost) if we apply a novel DSP similar to the one that was presented in~\cite{boutros2018embracing} and will be adopted in the next generation Agilex devices~\cite{Intel_agilex_dsp}.

\iffalse
\subsection{Data Quantization}\label{subsec:data_quant}
%Many previous efforts \cite{han2017ese, fowers2018configurable, rybalkin2020efficient, rybalkin2017hardware} have shown that RNNs/LSTMs are robust to low bit-width quantization. Instead of using double or single precision floating-point representation, fixed-point representation can be used in FPGA-based RNN accelerators to achieve high performance and high power efficiency. In this work, we convert the input vector, the hidden units and the weights to 8-bit integers. All arithmetic operations are performed in fixed point and our experiments demonstrate that there is no significant accuracy degradation with fine-tuning applied. To quantize and dequantize a real value $r$, we use the following affine mapping \cite{jacob2018quantization}:
%$r = S(q-z)$
There has been much previous work~\cite{han2017ese, fowers2018configurable, rybalkin2020efficient, rybalkin2018finn} demonstrating that RNNs are robust to low bit-width quantization. Fixed-point representation is often used in FPGA-based RNN accelerators which achieve higher performance and power efficiency than the ones using floating-point representation. This work quantizes the input vector, the hidden vectorand the weights into 8-bit integers. It performs all arithmetic operations in fixed-point. Our experiments show that there is no significant accuracy degradation with fine-tuning applied. To quantize and dequantize a real value $r$, we use the following affine mapping \cite{jacob2018quantization}: 
\begin{align*}
    r &= S(q-z)     \tag{2} \label{eq:2}
\end{align*}
where scale factor $S$ and zero point $z$ are the parameters of quantization. $S$ is a positive real number given by $(r_{max}-r_{min})/(q_{max}-q_{min})$, which scales the floating-point numbers to fixed-point integers. %$ \frac{r_{max} - r_{min}}{{q_{max}} - {q_{min}}} $. 
Note that ${r_{max}}$ and ${r_{min}}$ are maximum and minimum values of a real value respectively; $q_{min}$ and $q_{max}$ represent the range of an N-bit integer (e.g. 0 and 255 when N=8). The zero point $z$ denotes what value the real number zero represents in the quantized integer range. Please note that $S$ is a floating-point number whereas the zero-point is of the same type as the quantized value ($q$) which is an N-bit integer. However, modern implementations often bypass this floating-point multiplication by approximation techniques shown to have a negligible effect on the accuracy of the neural network. 
%In practice, data quantization is done off-line, and the accuracy loss brought by data quantization should be estimated and tested by the users of FP-DNN in advance. 

To avoid data overflow and maintain accuracy, the partial quantization \cite{fan2019f} is adopted to extend the bit-width of intermediate data. In this work, an 8-bit fixed-point data format is introduced to implement the multipliers in the Kernel units. All the 16-bit products of the multiplications are passed to the adder tree to preserve its accuracy, while the accumulators are 32-bit. 
The multipliers and adders for the element-wise operations in the LSTM-tail all use 16-bit fixed-point precision. 
%[GTC17] shows that the widely used NN models, including AlexNet, VGG, and ResNet50/100/152, can be quantized to 8 bit without inference accuracy loss using the same quantization scheme.
%Furthermore, quantization-aware fine-tuning~\cite{jacob2018quantization} is applied to our quantized RNN/LSTM to keep the accuracy. 
%\subsection{TODO: Combining the Sigmoid/Tanh and Quantization}
\fi




\section{Experimental results and Analysis}
This section introduces the experimental results on an Intel Stratix 10 FPGA which show the advances of the Remarn for RNN/LSTM accelerations. 

\subsection{Experimental Setup}

%For our study, we choose our benchmark workloads from the DeepBench suite \cite{fowers2018configurable, eriko_fccm19} for a fair and direct comparison. It is a set of micro-benchmarks containing representative layers from popular DNN models such as DeepSpeech \cite{deepspeech}. 
\tabref{table:benchmark} lists some benchmark workloads which are chosen from several typical LSTM applications to make a fair and direct comparison of our design with others. Multi-tasked LSTM workloads are constructed randomly from these LSTM workloads.
We evaluate the Remarn on an Intel Stratix 10 2800 (S10) and compare the results with other work. The Remarn runs the inferences of persistent LSTM models that store the weights in on-chip memory~\cite{fowers2018configurable, eriko_fccm19, que2020optimizing, que2020reconfigurable, rybalkin2018finn, rybalkin2020efficient, rybalkin2020massive}. Remarn is designed using Verilog RTL. And Quartus Prime Pro 19.4 is used for the compilation of FPGA designs. 

The choice of the number of sub-core is based on the size of the benchmark LSTM workloads and the accelerator hardware architecture.
The value of $EP$, explored in~\cite{que2020optimizing}, is set to 16, the same size as the previous designs~\cite{que2020optimizing, que2020reconfigurable}. 
The value of $VP$ should be chosen to be as large as possible. However, the largest effective value of $VP$ is $4L_h$ as discussed in~\secref{subsec:blocking}. Hence, the $VP=256$ in this work since the $L_h=64$ for the smallest LSTM benchmark as shown in~\tabref{table:benchmark}, resulting in $256\times 16=4096$ effective PEs for each sub-accelerator core. To make a fair comparison, the number of sub-accelerator cores, $N$, is set to 4 so that Remarn will have 16,386 PEs, which is the same as the number of total PEs in our previous designs~\cite{que2020optimizing, que2020reconfigurable}. 

\input{benchmark.tex} 

%We benchmark our implementations with the 6 benchmarks listed in Table 1. 
%Three of them are single-layer models and the other three are multi-layer models. 



\input{resources.tex}

\subsection{Resource Utilization}

Table \ref{table:utili} shows the resource utilization of our designs with two configurations on FPGAs. The first design is a baseline design which is a single-threaded design without partition. It utilizes the parameter of $(EP, VP)$ as (16, 1024), which includes 16,384 8-bit multipliers in the MVM kernels implemented using DSP blocks with extra ALMs. The second design is a dual-threaded quad-core Remarn which has 4 sub-accelerator cores. Each core utilizes the parameter of $(EP, VP)$ as (16, 256). Thus, it has the same number of multipliers as the baseline design. 
The dual-threaded quad-core design consumes 5.0\% more of total logic (ALMs) resources and 0.8\% more block ram (M20K) than the baseline design. Since dual threads share the same physical core it consumes the same DSP resources as the single-threaded one. 
%Although we achieve a similar frequency to which reported in the original BW paper \cite{fowers2018configurable} and Intel-NPU \cite{eriko_fccm19}, we believe that further low-level optimizations can be applied to our implementation to achieve even higher operating frequencies. We leave that for future work since it has a limited impact on the conclusions we draw from our study in this paper.
\input{cmp_cpugpu.tex}




\subsection{Performance and Efficiency Comparison with CPUs and GPUs}\label{subsec:to_gpu}
%To compare the performance of the proposed design on FPGA with other FPGA-based design, check Table \ref{table:laten} and Fig. \ref{fig:utz_lstm}, Fig. \ref{fig:utz_gru}.

To compare the performance of the proposed design on FPGA with other platforms, the DeepBench published results~\cite{zhao2019serving} on an Intel Xeon Syklake CPU and NVIDIA Tesla V100 GPU are used for comparison. TensorFlow is used for both CPU and GPU. 
%The AVX2 vector instructions are enabled for the CPU while the CuDNN libraries are enabled for the GPU. 
Besides, the CPU with AVX2 Vector instructions enabled is utilized while the CuDNN libraries are enabled for the GPU. cuDNN is a GPU-accelerator Library from NVIDIA, which is specialized for deep learning. 
%The LSTMBlokcFusedCell kernels in TensorFlow are used for evaluation. 
Both CPU and GPU implementations run with a batch size of 1, which provides the lowest service latency of cloud since requests are required to be processed as soon as they arrive. For a fair comparison with the throughput of our dual-threaded Remarn, the throughput of the CPU and GPU have been doubled in~\tabref{table:cpugpu}. The GPU is significantly underutilized even when cuDNN library API calls, since it is designed for throughput-oriented workloads. It prefers BLAS level-3 (matrix-matrix) operations that are not common in RNN computations~\cite{zhao2019serving}. 
%Compared with the RNN/LSTM running on GPU, our FPGA design of STM-LSTM is 6.53 times faster and 15.69 times higher power efficiency respectively as shown in~\tabref{table:cpugpu}.
Our FPGA design of dual-threaded Remarn achieves 6.5 times higher performance and  15.6 times higher power efficiency respectively than the one running on the Tesla V100 GPU as shown in~\tabref{table:cpugpu}.



\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.8\linewidth]{img/Speedup_t05.pdf}
\end{center}
   \caption{Performance speedup for quad-core Remarn with various threads.}
\label{fig:speedup}
\end{figure}


\subsection{Performance and Efficiency Comparison with the baseline}\label{subsec:to_baseline}

To show the benefits of the proposed approaches, we compare the multi-threaded multi-core Remarn with the baseline design~\cite{que2020optimizing} in~\figref{fig:speedup} and~\figref{fig:utilization}. The baseline is a single-threaded single-core accelerator. 
Hardware utilization is the percentage of the peak Tera Operations Per Second (TOPS) achieved for each LSTM, as compared with the peak TOPS of the design with all the PEs. %The mixed multi-tasked LSTM workloads are constructed randomly from these LSTMs. 
\figref{fig:speedup} shows the speedup of the quad-core Remarn over the baseline design~\cite{que2020optimizing}. 
%With the proposed approaches of CGMT and multi-core, the quad-core Remarn design of quad threads (4-T-Q) achieves 14.44 times higher performance than the baseline~\cite{que2020optimizing} when targeting the small LSTMs ($h=64$). 
With the proposed approaches of CGMT and multi-core, the quad-core Remarn designs of a single thread (1-T-Q), dual threads (2-T-Q) and quad threads (4-T-Q) achieve 1.82, 2.91 and 3.16 times higher performance respectively than the baseline when targeting mixed requests from LSTM workloads with $h=64,128$ and $256$. 
Please note that Remarn has the same number of PEs as the baseline, and they consume the same DSP blocks on FPGAs. 
%The quad-core Remarn of a single thread (1-T-Q), dual threads (2-T-Q) and quad threads (4-T-Q) achieve 1.82, 2.91 and 3.16 times higher performance respectively than the baseline when targeting mixed requests from LSTM workloads with $h=64,128$ and $256$.
%These designs utilize the same number of 8-bit multipliers in the MVM kernels. 
%With 4-thread, it achieves 2.23 times higher than the single thread core using the same computational engines. 
Particularly, with 4 threads (4-T-Q), Remarn achieves 14.44 times higher performance than the baseline~\cite{que2020optimizing} when targeting the small LSTMs ($L_h=64$). 

When only targeting large LSTMs, the performance gain of the quad-core Remarn is small since the baseline design~\cite{que2020optimizing} already achieves high hardware utilization for these LSTMs. 
%As illustrated in \figref{fig:speedup}, Remarn get more or less the same performance as the baseline when targeting the LSTMs with $h=512$.
However, the baseline still suffers from low utilization when targeting small-sized LSTMs which are commonly used in many applications~\cite{peng2019exploiting, lrcn_donahue2015long}. LSTM models which have a large number of timesteps but use small sizes are the most tangible examples which require dealing with lots of dependencies, as well as the parallel task of MVMs~\cite{yazdani2019lstm}. Our proposed approach and hardware architecture can alleviate this problem by leveraging the coarse-grained multithreading combining the spatial co-execution using multiple sub-accelerator cores. 
With the demand for high-performance designs, it is vital to maximize the hardware utilization to attain the best possible effective performance and power efficiency. 



\begin{figure} 
   \centering
  \hspace*{\fill}
  \subfloat[\label{fig:utilizationa}]{%
    \includegraphics[width=0.48\linewidth]{img/utilization_mt_t01.pdf}}
  \hfill
  \subfloat[\label{fig:utilizationb}]{%
    \includegraphics[width=0.48\linewidth]{img/utilization_q01.pdf}}
    
  \caption{Hardware utilization targeting various LSTM tasks. (a) Hardware utilization of different LSTM tasks using various threads with a single big accelerator. (b) Hardware utilization of different LSTM tasks using various threads with 4 sub-accelerator cores.}

  \label{fig:utilization} 
\end{figure}

\begin{figure}%[ht]
\begin{center}
\includegraphics[width=0.7\linewidth]{img/Speedup_f_t05.pdf}
\end{center}
   \caption{Performance speedup of the multi-threaded quad-core Remarn over the multi-threaded single-core design.} 
\label{fig:speedup_f}
\end{figure}


When compared to our previous work~\cite{que2020reconfigurable} with only multithreading, Remarn can attain much higher hardware utilization and performance. Remarn achieves higher than 50\% utilization for all the LSTM cases with $L_h=128$ as shown in~\figref{fig:utilizationb} while the previous work can only achieve up to 36.4\%. Particularly, With dual threads, the previous work achieves the utilization lower than 25\% for LSTMs with $L_h=128$, however, the proposed Remarn can achieve higher than 75\%. 
%It is much higher than the one of our previous 4-thread design~\cite{que2020reconfigurable}, which is lower than 25\%. 
%\figref{fig:utilization} illustrates that Remarn achieves much higher hardware utilization than our previous design~\cite{que2020reconfigurable} without fission, especially targeting small LSTM workloads. 
%while it is able to maintain the performance for large LSTMs. 
Compared to our previous work~\cite{que2020reconfigurable}, the Remarn proposed in this work achieves up to 3.61 times higher performance when targeting the small LSTMs, as shown in~\figref{fig:speedup_f}, which shows the advances of the proposed architecture using multiple sub-accelerator cores. 
There is a small reduction from a linear speedup for the model size of 64, which is due to control logic added to each small cores when splitting the big engine. The impact is negligible when the workload is large with a long run time. We believe this can be optimized with more efforts but doing so has little impact on the conclusions we draw from this study. 

The design with multithreading alone shows a steady increase from 1-T to 2-T and to 4-T~\cite{que2020reconfigurable} for the model size of 128. However, the additional speedups for the quad-core design dropped when it is from 2-T to 4-T threads as shown in~\figref{fig:speedup_f}. It is because with 2-T on small cores, the design can already remove most of the stalls caused by the RNN data dependencies for the model size of 128. Hence, the quad-core design with 2-T and 4-T achieves a similar performance and runtime hardware utilization as shown in~\figref{fig:utilizationb}. But with 2-T on the big core, the design still suffers from some stalls so the performance of 4-T on the big core is much better than 2-T. Hence, the additional speedups drop when going from 2-T to 4-T threads on the quad-core design. 

Morevoer, when compared to~\cite{que2020optimizing, que2020reconfigurable} which has a single large core, the quad-core Remarn has a slight performance drop (less than 2\%) when all 4 cores are working together as a big accelerator to run a large workload, as shown in~\tabref{table:cpugpu} and~\tabref{table:cmp}. 
It is because the multi-core design can lead to synchronization costs than the one using a monolithic accelerator. When four cores are running the same large workload, a synchronization mechanism is required to maintain the correct data dependencies in RNNs. It is a design trade-off. With slight performance loss on the large workloads, the design can achieve much higher performance on the small workloads, which can result in a much better performance gain for all the workloads. 
Besides, the users can re-configure the FPGA into a big and monolithic accelerator when most of large RNN workloads are large, which can achieve the best performance.   

The evaluation results also show that Remarn gets a low utilization when running small LSTMs ($h=64$), as shown in~\figref{fig:utilizationb}. Even with 4 threads, the design still stalls because the cycles of processing MVMs in the other threads still cannot completely hide the whole pipeline latency to get the $h_t$ available before it is required for the next timestep. The number of cycles to process the MVM of the LSTM gates is given by $\frac{Lx+Lh}{EP}$. 
%It is because the largest effective $VP$ in this case is $4 \times {Lh}$ which is $512$ so that the effective PEs are less than $NPE$, which leads to severe underutilization. 
Different choices of ($EP$,$VP$) impact the performance and utilization of the designs that run LSTMs with different sizes. There is a trade-off between the extra performance that can be achieved and the hardware design complexity as well as extra hardware resources of supporting various sets of ($EP$, $VP$) at runtime. It is our future work to enhance this accelerator architecture to support various sets of ($EP$, $VP$) since different sizes of LSTMs may prefer different optimal $EP$ and $VP$ parameters.

\input{cmp3.tex}

\subsection{Performance and Efficiency Comparison with other FPGA-based designs}\label{subsec:to_fpga}
\tabref{table:cmp} shows the comparison between our Remarn and the existing LSTM accelerator implementations using a Stratix 10 GX 2800 FPGA.  
For a fair comparison, we only show the previous work with a detailed implementation of the LSTM system using the same FPGA. We list the model storage, precision, DSP used, runtime frequency, power, throughput and power efficiency as well as the hardware (HW) utilization. The thermal design power (TDP) which is 125W is utilized for a fair comparison since it is reported in all the listed work. 
%Hardware utilization is the percentage of run time during which the hardware is not idle. 
%With a similar number of DSP resources to \cite{eriko_fccm19}, our design achieves 94.1\% hardware utilization which is the highest with respect to state-of-the-art implementations on FPGAs, as shown in \figref{fig:utz_lstm} and \figref{fig:utz_gru}. 
%The GPU is underutilized with only 0.4\texttildelow3\% \cite{fowers2018configurable} of its peak TOPS. 
Overall, Remarn provides over 4.87 times higher performance and 5.71 times higher hardware utilization than the SOTA design~\cite{eriko_fccm19} when targeting LSTM models with $h_t$=256, as shown in~\tabref{table:cmp}. Compared with the baseline which is a single-threaded single-core design~\cite{que2020optimizing}, Remarn achieves 1.45 to 14.4 higher throughput and HW utilization.
%These design~\cite{fowers2018configurable, eriko_fccm19} do not report the performance of LSTMs with $h < 256$. 
Since multithreading also ensures there is no downside to peak performance in a single-threaded mode, the Remarn can achieve a similar peak performance with the one in~\cite{que2020optimizing}, which is the highest with respect to the SOTA FPGA-based RNN/LSTM designs with a commonly used INT8 precision. The only prior work that has a higher peak performance is~\cite{fowers2018configurable} which employs an 8-bit block floating-point representation. However, when targeting the small LSTM models, the throughput of the proposed Remarn is 18.82 times higher than~\cite{fowers2018configurable} as shown in~\tabref{table:cmp}. Moreover, Remarn achieves the highest hardware utilization among all the listed designs across various LSTM models. This work focuses on maximizing throughput and minimizing latency by increasing HW utilization. 
%The proposed Remarn architecture improves the efficiency of hardware usage from another point of view, hence it accelerates the effective performance. %not peak one. 

%When $h=256$, We do not get a high hardware utilization like other cases. It is because the cycle of $Lx/EP=16$ is too small to fully hide the data-dependency. However, with our novel hardware architecture and tiling strategy, we can still process 
%In addition, our design achieves on average 1.35x and 1.39x better performance and energy efficiency than \cite{eriko_fccm19} respectively. 
%The results show flexible customizability of our architecture for different scenarios.


%although they demonstrate diverse multi-DNN scheduling optimizations are effective at meeting the restricted latency requirements and increasing the hardware utilization, they fail to handle the simultaneous execution of multiple DNN models and thus cannot obtain the optimal performance under SMT supports and decoupled architectures.

%\vspace{-0.5cm}
\subsection{Scheduling}\label{subsec:to_fpga}
The scheduling strategy for multi-core accelerators for DNN workloads is a new and rarely explored topic. PREMA~\cite{choi2020prema} introduces a preemptive scheduling algorithm on a single-core NPU to support multi-DNN execution. AI-MultiTasking~\cite{baek2020multi} proposes to process different neural networks by partitioning their various layers into identical sub-layers in compile time. It also develops a heuristic of mapping DNN jobs to the accelerator. 
%It exploits three scheduling mechanisms, including First-In-First-out (FIFO), Round-Robin (RR), and greedy algorithm. The RR scheduling repeatedly selects one sub-layer from different neural networks. 
In~\cite{kwon2021heterogeneous} Heterogeneous Dataflow accelerators (HDAs) are proposed to support the heterogeneous acceleration of multi-DNN workloads using manual-designed mapping of jobs to sub-accelerators and compile time layer-wise scheduling. LayerWeaver~\cite{oh2021layerweaver} introduces a layer-wise time-multiplexing scheduler on single NPU by interweaving layer execution to increase the hardware utilization. Besides, MAGMA~\cite{kao2022magma} proposes a novel framework for mapping multiple DNNs on multiple accelerator cores. 


The focus of this paper is on the accelerator architecture, and on examples of optimal utilization of that architecture based on fine-grained scheduling of tasks made up of LSTM sub-layers running on sub-cores. We exploit the intra-model data dependencies of both timesteps and layers in LSTMs, as shown in~\figref{fig:lstm_layers}(a). Both time step and layer dependencies have a linear dependence chain in the model. For LSTM inference, it is processed from the first layer to the last layer sequentially and from the first timestep to the last timestep in each layer. Besides, layers from different LSTMs are independent. Inspired by~\cite{baek2020multi, kwon2021heterogeneous} which rely on manually-designed heuristics, this work develops a set of heuristics which exploit the characteristics of LSTM inference workloads to reduce the scheduling overhead for the proposed homogeneous multi-core accelerator. 
We do not include algorithmic details (e.g. flowchart or pseudocode) about scheduling of these sub-layers tasks, other than mentioning related research on scheduling strategies~\cite{choi2020prema, baek2020multi, kwon2021heterogeneous} and LayerWeaver~\cite{oh2021layerweaver} as well as the custom mapping algorithm MAGMA~\cite{kao2022magma}. 
Architectural tradeoffs of these scheduling strategies, based on queuing theory and other techniques, are important and would be best addressed by future work. Besides, further research will cover fine-grained dynamic scheduling for our accelerator, such as using Gang scheduling which schedules a gang of jobs onto free cores. Furthermore, other sophisticated scheduling strategies relevant to our approach will be studied and tested. 


%We do not include algorithmic details (e.g. flowchart or pseudocode) about static or dynamic scheduling of such tasks, other than mentioning related research on scheduling strategies~\cite{choi2020prema, baek2020multi, kwon2021heterogeneous} and LayerWeaver~\cite{oh2021layerweaver}. Architectural tradeoffs of these scheduling strategies, based on queuing theory and other techniques, are important but would be beyond the scope of this paper. 

\subsection{Power Consumption and Optimizations}

%Generally, adding new cores will increase the power consumption. However, our design is not adding new big cores. 
The proposed extension of the multi-core feature is based on splitting a large monolithic accelerator into several sub-accelerator cores, which does not change the total number of existing PEs in hardware. There is only a small bump in the hardware resources for the extended accelerator because of supporting new features, which may cause a little more power/energy consumption. However, the extra power consumption caused by extra FPGA hardware resources is small 
since the new design only has 5\% more area than the baseline~\cite{que2020optimizing} but can get 1.45 to 14.4 times higher performance, resulting in high power efficiency
%since the new design only has 5\% more area than the baseline~\cite{que2020optimizing}. But we can get much higher performance, resulting in higher power efficiency.



Besides, the architectural extensions lead to higher runtime dynamic power since these extensions provide more parallelism and higher hardware utilization. In general, the performance and power are positively correlated;  the more accelerators used, the higher the power consumption. However, higher utilization also means that our architecture wastes less power on the underutilized execution resources than the baseline~\cite{que2020optimizing}, which increases the overall power/energy efficiency. The overall increase in utilization also means the proposed design completes the same work in a shorter period of time, resulting in a potential lower energy consumption. Besides, with multiple sub-accelerator cores, the design has the potential to totally turn off some of the cores when there is only a small amount of workload to save power, which is not possible in the baseline where only a big and monolithic core is used. In future work, we will build an architecture-level power model targeting multi-threaded multi-core DNN accelerators so that we can quantify the impact of these architectural extensions on power/energy consumption. 




There are some potential optimizations for the power consumption targeting our architecture. Since the proposed design achieves a high hardware utilization, it may not require so many PEs to reach a design performance goal. Reducing the number of total PEs or reducing the hardware resources in design time can help to reduce the total power consumption. On the other hand, the design causes large dynamic power consumption because of the high utilization. Hence, one possible optimization is to control dynamic power consumption by gracefully degrading the core activities when a power consumption threshold is exceeded. It can be done by a feedback of the current power consumption of the cores, which may be estimated from some performance counters or read from some on-die sensors.  



%\vspace{0.5cm}

\section{Related Work}

%\subsection{Previous Work}\label{sec: previous}
There are many previous studies about FPGA-based accelerations of persistent RNN/LSTM with weights stored in on-chip memory~\cite{rybalkin2017hardware, fowers2018configurable, eriko_fccm19, que2019aelstm, rybalkin2018finn, rybalkin2020efficient, rybalkin2020massive}. 
Rybalkin et al.~\cite{rybalkin2017hardware} introduces the hardware architecture of BiLSTM targeting OCR applications. All the weights and activations are quantized to 5-bit and stored in on-chip memory. \cite{rybalkin2018finn} quantizes the design using 1-8 bits and achieves an accuracy which surpasses the one using floating-point on a given dataset. Besides, their later work~\cite{rybalkin2020efficient, rybalkin2020massive} proposes a novel hardware architecture of 2D-LSTM and investigates the trade-off between precision and performance. 
%Many studies are focusing on weight pruning and model compression to reduce the size of weights and input activations~\cite{han2017ese, gao2018deltarnn, cao2019efficient, shi2019lstm}. 
There are also many previous studies about LSTM implementations with weights stored in off-chip memory on FPGAs~\cite{guan2017fpga, chang2015recurrent, guan2017fp, park2020time, que2019efficient}, which has been recognized as the performance bottleneck. 
%since the fetched weights are typically used only once in each LSTM timestep computation. 
In LSTM computations, a weights matrix tends to be repeatedly loaded from off-chip memory if the size of on-chip memory is not large enough to store the entire matrix, which brings large latency. Guan et al.~\cite{guan2017fpga} proposes a smart memory organization with on-chip double buffers to overlap computations with data transfers. 
%And~\cite{gao2018low, ardakani2018learning, silfa2020batch}
And~\cite{gao2018low, silfa2020batch} apply the batching technique to increase the throughput of LSTM inferences. E.g., E-BATCH is proposed~\cite{silfa2020batch} for RNNs, which increases throughput while also improving energy efficiency on an ASIC-based accelerator.
Apart from batching, \cite{que2019efficient, park2020time, que2020mapping} introduce novel LSTM weights reuse schemes which utilizes the weights sharing characteristics in different timestep computations in one inference. These schemes reduce the access of the off-chip memory and decrease the energy cost as well as improve the design throughput. 

Some of the previous work~\cite{wang2017accelerating, wang2018c, li2019rnn, yalamarthy2019low} adopts circulant matrix to optimize LSTMs by reducing the weight matrices of LSTM inferences. 
Besides, an approximate computing scheme is deployed for LSTMs using small tiles~\cite{rizakis2018approximate}. And stochastic computing is used to improve the energy efficiency of the RNN inference~\cite{liu2019energy}. \cite{khalil2021reversible} proposes an LSTM architecture based on reversible logic gates for low power circuit designs. 
%\cite{chen2020blink} proposes BLINK which utilizes bit-sparse data representation for LSTM inferences. 
POLAR~\cite{bank2019polar} and BRDS~\cite{ghasemzadeh2021brds} present FPGA-based pipelined and overlapped architecture for dense and sparse LSTM inferences respectively.
%In~\cite{que2019aelstm} a novel Timestep(TS)-buffer is introduced to avoid redundant calculations of LSTM gate operations to reduce system latency. 
A multi-FPGA approach~\cite{sun2019acceleration} is proposed to accelerate multi-layer RNNs. It achieves a single-layer latency targeting deep RNNs with arbitrarily multiple layers using an FPGA-based cluster.
\cite{nurvitadhi2019scalable} presents a multi-FPGA based architecture to accelerate neural machine translation. 
\cite{kwon2020scalable} explores various partitioning strategies of large RNN inferences to achieve scalable multi-FPGA acceleration. It also analyses the performance impact of software pipelining and collective communications. 
PDL-FGPU~\cite{ma2021specializing}, a specialized FPGA-based GPU overlay architecture is proposed to run persistent Deep Learning, including various RNN variants. Initiation interval (II) balancing~\cite{que2021accelerating} is proposed with a layer-wise implementation of LSTMs to achieve ultra low latency. The layer-wise implementation of RNNs is also used in accelerating Bayesian RNNs~\cite{ferianc2021optimizing}. 

%~\cite{nan2020dc}
There is also much previous work~\cite{han2017ese, chen2018clink, gao2018deltarnn, wu20193, cao2019efficient, shi2019lstm, nan2020dc,chen2020blink, zheng2021permlstm, gao2021spartus, jiang2022low} exploit the sparsity of data and weights with pruning to reduce the NN computation and also the memory footprint to achieve high performance and efficiencies. ESE~\cite{han2017ese} proposes a pruning technique that compresses a large LSTM model by 20$\times$ without sacrificing the prediction accuracy. DeltaRNN~\cite{gao2018deltarnn} utilizes the Delta Network algorithm to reduce MxV operations and corresponding weight fetches by skipping dispensable computations during inference of RNNs. It updates the output of a neuron only when the neuron’s activation changes by more
than a delta threshold.
BBS (Bank-Balanced Sparsity)~\cite{cao2019efficient} is proposed to achieve both high prediction accuracy of a pruned LSTM model and high hardware efficiency of the model running on FPGAs. It partitions weight matrix rows into banks for parallel computing and adopts fine-grained pruning inside each bank to maintain model accuracy.
BLINK~\cite{chen2020blink} designs the LSTM inference using a bit-sparse data representation. And it turns multiplications into bit-shift operation to improve the energy efficiency while maintaining the LSTM inference accuracy for real-time calcium image processing. The extension~\cite{chen2022energy} proposes a combination of the bit-sparse quantization and the pruning methods for energy-efficient LSTM inferences. 
More recently, Spartus~\cite{gao2021spartus} exploits spatio-temporal sparsity to achieve ultra-low latency inference using Column-Balanced Targeted Dropout (CBTD). These studies are orthogonal to our proposed approach and hardware architecture. These techniques can be complementary to our approaches to achieve even higher performance and efficiency of RNN/LSTM inferences using FPGAs. 


The Brainwave design \cite{fowers2018configurable} is a single-threaded SIMD architecture for running real-time AI, including persistent RNNs. It achieves more than an order of magnitude improvement in latency and throughput over state-of-the-art GPUs on large memory intensive RNN models at a batch size of 1. It stores NN model weights on-chip for RNNs to get a necessary high memory read bandwidth to achieve higher performances. A coarse-grained reconfigurable architecture (CGRA) based RNN accelerator is proposed~\cite{zhao2019serving} on top of Plasticine~\cite{prabhakar2017plasticine} with a set of techniques for performing cross-kernel optimization in RNN cells. 
AERO~\cite{kim2021aero} is a single-threaded instruction-set based processor using a versatile vector-processing unit customized for RNN inferences on resource-limited FPGAs. 
A Brainwave-like neural processing unit (NPU) is proposed in~\cite{eriko_fccm19} with a single-threaded architecture. They also explore the potential of combining a TensorRAM with FPGAs to provide large high-speed memory for large memory intensive RNN sequence models. Besides, their late work~\cite{boutros2020beyond} deploys the Brainwave-like NPU on the Stratix 10 NX which is Intel’s new AI-optimized FPGA featured with AI tensor blocks. \cite{que2020optimizing, que2022recurrent} proposes a novel latency-hiding hardware architecture based on column-wise MVM and fine-grained tiling strategy to eliminate data dependency of RNNs, which improves the design throughput of RNNs/LSTMs. However, all these NPUs targeting RNNs/LSTMs are single-threaded. 

There is a large demand for architectural support of multi-DNN execution to maximize hardware utilization and reduce the costs of a large-scale production system. E.g., TensorRT from Nvidia supports concurrent DNN execution for users to run multi-DNN workloads on the same GPU simultaneously. 
%While~\cite{baek2020multi} proposes AI-MT, which fully utilizes the accelerator’s computation resources and memory bandwidth by matching compute- and memory-intensive tasks from different networks and executing them in parallel using memory block prefetching and compute block merging. There is a flow proposed in~\cite{nurvitadhi2010automatic} to auto-generate multi-threaded processing pipelines. \cite{peng2019exploiting} proposes a dual-core accelerator for LSTM-RNN, which is able to execute multiple jobs simultaneously or have cores collaborate on a single job. However, they utilize the dual-core with each thread running on each core. It will half the performance if there is only one task, which is not efficient. 
%There are some previous work on DNN accelerator using multireading. 
SMT-SA~\cite{shomron2019smt} presents a simultaneous multithreading approach for systolic arrays to solve the issue of underutilization because of zero-valued inputs. However, it is not able to deal with the underutilization issue that comes from the data dependencies in RNNs/LSTMs.
A multi-threaded CGRA~\cite{ando2017multithreaded} has been proposed, but it is only for CNN accelerations. %\cite{nurvitadhi2010automatic}~introduces a synthesis technique to auto-generate in-order multi-threaded processing pipelined datapath using the high-level specification of an unpipelined datapath. 
\cite{nurvitadhi2010automatic}~presents to generate in-order multi-threaded processing pipelined datapath automatically with the high-level specification of an unpipelined datapath.
CUSTARD~\cite{dimond2006application} presents a customisable multi-threaded FPGA soft processor with features including design space exploration and a compiler for automatic selection of custom instructions. 
More recently, PREMA~\cite{choi2020prema} proposes a preemptible NPU with a preemptive scheduling algorithm to support multi-DNN execution. However, it does not consider the data dependencies between RNN/LSTM timesteps. %The sequence length (timestep) of an LSTM model is usually larger or much larger than the number of layers.
AI-MultiTasking~\cite{baek2020multi} proposes to balance memory-intensive and compute-intensive tasks from different neural networks and process them in parallel by partitioning various layers into lots of identical sub-layers. The RNNs are handled just as FC layers in the scheduling scheme. However, RNNs are more complex than FC layers that have no data dependencies. 
In~\cite{peng2019exploiting}, 
a dual-core accelerator for LSTM-RNN is proposed to execute multiple jobs simultaneously or have cores collaborate on a single job. However, they perform multithreading by utilizing the dual cores with one thread on one core, which is not an area~/~cost efficient way to add extra threads.
%This affects the design performance in a single thread mode since they can only use half of the computational resources to run a single task.
Besides, there is some previous work targeting spatial multi-tenant execution. f-CNN$^x$~\cite{venieris2018f} employs multiple custom dedicated engines for the workloads with various CNN models. \cite{ribes2020mapping} maps multiple LSTM models to an FPGA device by introducing a framework that alters their computational structure, opening opportunities for co-optimizing the memory requirements to the target architecture via applying compression schemes across multiple LSTM models.
In~\cite{kwon2021heterogeneous} Heterogeneous Dataflow accelerators (HDAs) are proposed to support the heterogeneous acceleration of multi-DNN workloads. 
More recently, Planaria~\cite{ghodrati2020planaria} introduces the dynamical fission of a systolic-array based DNN accelerator at runtime to support spatial co-execution of multiple DNN inferences. However, none of them targets RNNs, and they do not consider the recurrent nature and data dependency in RNN computations. This work designs a multi-threaded accelerator with fission to enable spatial and temporal co-execution of multiple RNN/LSTM inferences on the same hardware and offers simultaneous multi-RNN accelerations. It can handle multiple requests using multi-threaded mode with multiple sub-accelerator cores while still being able to run a task in a single-threaded mode with a large accelerator to attain higher performance and lower latency when targeting the workloads with high priority.  

%A primary goal of our design is to efficiently add more per-NPU core scalability potential. 

%The multi-core technique can be complementary to our approach to achieve even higher throughput of RNN inferences on FPGAs. 


%Furthermore, it will be easy to extend our approach to multi-core accelerators to further improve the performance using more hardware resources. 

%METRO~\cite{wang2021metro} is proposed to improve the efficiency of the interconnections in the tile-based architectures by decoupling the traffic scheduling policies from hardware fabrics and moving them to the software level. 






\section{Conclusions and Future Work}

This work proposes Remarn, a multi-threaded multi-core neural processing unit (NPU) supporting spatial and temporal co-execution of RNN/LSTM inferences to improve the processing abilities of cloud-based NPUs. The Remarn can increase the throughput while improving the hardware utilization of the cloud-based NPUs.
%the processing abilities of cloud-based NPUs to reduce latency and improve hardware utilization to boost system performance. 
We have implemented the proposed multi-threaded multi-core accelerator architecture on Intel Stratix 10 FPGAs with superior performance and efficiency, which demonstrates the effectiveness of our approaches. 
Our study shows that both multithreading and multi sub-accelerator core techniques can address the underutilization issue (resource inefficiency) when targeting small sized RNN workloads. Besides, it also shows that multi sub-accelerator core is slightly better than multithreading for small workloads. The design of quad-core with single-thread (1-T-Q) achieves a better utilization than the design of single-core quad-thread (4-T) for the LSTM of $L_h=128$, as shown in~\figref{fig:utilization}. But this figure also shows that the single-core quad-thread (4-T) design gets a better performance for the LSTM of $L_h=256$. In addition, both techniques do not bring benefits to large LSTM workloads since the baseline design has achieved high utilization. 
Moreover, this study shows that multithreading targets temporal co-execution , while multi-core targets spatial co-execution, and the two techniques can be combined to achieve a much better performance. 
%Further research includes combining our method with simultaneous multithreading (SMT) and the automation of the proposed approach to enable rapid development of efficient RNN/LSTM designs.
Further research includes exploring how Remarn can benefit from other enhancements such as dynamic scheduling and runtime power analysing, studying the trade-offs of varying the number and the heterogeneity of Remarn cores, and automating the proposed approaches to enable rapid development of efficient Remarn designs for datacentres as well as edge processing and embedded systems. 



\begin{acks}
%\textbf{Acknowledgement:}
The support of the United Kingdom EPSRC (grant numbers EP/V028251/1, EP/L016796/1, EP/N031768/1, EP/P010040/1, and EP/S030069/1), Corerain and Intel is gratefully acknowledged.

\end{acks}

%\section{To Read}
%https://ieeexplore.ieee.org/abstract/document/8906688

%Exploiting Model-Level Parallelism in Recurrent Neural Network Accelerators




==> resources_t.tex <==
\begin{table}%[b]
\centering
\caption{Resource utilization.}
\label{table:utili}

\scalebox{0.95}{\begin{tabular}{ c | c | c |c| c| c}
\toprule
 \multirow{2}{*}{\textbf{Task}} & & \textbf{LUT}   & \textbf{FF}  & \textbf{BRAM} & \textbf{DSP}\\
\cmidrule{2-6}
 &  \textbf{Available} & 1728k & 3456k & 5376 & 12288  \\
\midrule
JEDI-net 30P  & Used [$\downarrow$] &  1158k &  246k & 1392 & 11504 \\ \cmidrule{2-6}
(\textbf{J2~\cite{que2022optimizing}}) & Utiliz. [\%, $\downarrow$] & 67 &  7.1 & 25 & 93  \\
\midrule
JEDI-net 30P  & Used [$\downarrow$] &  734k &  137k & 16 & 9013 \\ \cmidrule{2-6}
(\textbf{J3, w/ fusion}) & Utiliz. [\%, $\downarrow$] & 42 &  4.0 & 0.3 & 73  \\
\midrule
\midrule
JEDI-net 30P  & Used [$\downarrow$] &  865k &  138k & 37 & 7267 \\ \cmidrule{2-6}
(\textbf{J4}, Opt-Latn) & Utiliz. [\%, $\downarrow$] & 50 &  4.0 & 0.7 & 59  \\
\midrule
JEDI-net-30P  & Used [$\downarrow$] &  911k &   153k & 37 & 9833 \\ \cmidrule{2-6}
(\textbf{J5}, Opt-Acc) & Utiliz. [\%, $\downarrow$] & 53 &  4.4 & 0.7 & 80  \\
\midrule
JEDI-net-50P  & Used [$\downarrow$] &  855k &  201k & 25 & 8945 \\ \cmidrule{2-6}
(\textbf{U4}, Opt-Latn) & Utiliz. [\%, $\downarrow$] & 49 &  5.8 & 0.5 & 73  \\
\midrule
JEDI-net-50P  & Used [$\downarrow$] &  815k &   189k & 37 & 8986 \\ \cmidrule{2-6}
(\textbf{U5}, Opt-Acc) & Utiliz. [\%, $\downarrow$] & 47 &  5.5 & 0.7 & 73  \\
\bottomrule
\end{tabular}}
\vspace{0.2cm}
\end{table}

==> temp.tex <==
\section{backup}
\subsection{Task-level parallelism}
We categorize optimizations into two classes: intra-task and inter-task optimizations. 
Since each task is a separate unit, dedicated intra-task optimization can be applied to each task, such as outer-product based MMM (Section~\ref{sec:outer_mmm}) and exploiting structured sparsity of adjacency matrices (Section~\ref{sec:sparsity}).  
In addition, inter-task optimizations are also introduced for optimizing multiple tasks and their interactions, such as column-major order representation (Section~\ref{sec:cm}) for increasing the data spatial locality of intermediate results exchanged between different tasks, initiation interval balancing (Section~\ref{sec:iib}) for optimizing the overall initiation interval across multiple tasks, and a fusion technique (Section~\ref{sec:fuse}) for fusing multiple tasks to remove extra boundaries, reducing end-to-end latency. Moreover, a GNN-specific co-design approach (Section~\ref{sec:co-design}) is proposed to optimize the algorithm and hardware simultaneously, which produces more optimised designs such as DNN1, while maintaining model accuracy and achieving low design latency. By combining these different optimizations, the design can achieve good performance and efficiency.

\textcolor{\mycolor}{
%Although this work targets a GNN application, the proposed optimization techniques can be adapted to optimize other low latency designs for accelerating neural networks using a dataflow architecture.
%The specific GNN layered structure and coefficients are CERN LHC specific, but the proposed solution can be adapted to a different network to achieve low latency, such as the task-level parallelism based dataflow architecture and inter-task optimizations. These optimizations for low latency would benefit many other applications on FPGAs.  
The proposed GNN layered structure and coefficients are CERN LHC specific, 
%but the proposed solution of task-level parallelism based dataflow architecture 
while the dataflow architecture with task-level parallelism and the optimizations, especially the inter-task ones, can be adapted to other GNN networks or even to other types of neural networks. The optimizations for low latency can benefit many other applications on FPGAs, especially those that require real-time processing. 
%We propose several optimizations for the tasks and also the interactions between tasks to achieve high performance and efficiency designs. 
}


\subsection{Balancing initiation interval (II)}
\textcolor{\mycolor}{
A GNN model is composed of many components that use loops to execute repetitive algorithms for processing blocks of data, such as nodes and edges. 
To achieve high throughput and low latency, these loops can be unrolled, resulting in multiple copies of the loop body in hardware, allowing multiple or all loop iterations to occur in parallel. 
This can decrease the latency at the expense of additional hardware resources.} However, a naive implementation often results in an unbalanced \textcolor{\mycolor}{initiation interval (II)} in the coarse-grained pipeline, which causes hardware inefficiency and low system throughput. The II is decided by the largest II among all the units on the datapath. Generally, it is unnecessary to unroll every unit in order to achieve the lowest II. 
However, some hardware resources can be saved from the units that do not require full unrolling and then these resources can be re-allocated to the bottleneck unit that dominates the whole design to reduce the II of the design as well as the latency. 
Partitioning FPGA resources to enhance throughput/latency in a layer-wise architecture has been studied for CNNs~\cite{shen2017maximizing, zhang2020dnnexplorer, zhang2018dnnbuilder, gong2018maloc} and RNNs~\cite{que2021accelerating}, but there is little work focusing on GNNs. This work balances the IIs of the sub-layer units in GNNs by partitioning the FPGA resources appropriately. A design space exploration is also performed to find the appropriate parallelism parameters to achieve an optimal trade-off between the II and hardware resources. 




\begin{figure}
\begin{center}
\includegraphics[width=0.7\linewidth]{img/sr_reduction_t02.pdf}
\end{center}
   \caption{The reduction in the number of multiplications, additions and iterations for (a) MMM1/2 as well as (b) MMM3 of JEDI-net-30p models, and (c) MMM1/2 as well as (d) MMM3 of JEDI-net-50p models.}
\label{fig:sr_reduction}
\end{figure}
\subsubsection{\textbf{Optimization of custom code transformation}}
%The strength reduction removes all the multiplications in all three MMM units. Besides, when doing the inner product of each row vector of input $I$ matrix and each column vector of $R_r$ (or $R_s$) in MMM1/2, there is only one non-zero product. Thus, only load and store operations are required to compute $B1=IR_r$ as well as $B2=IR_s$. %Moreover, the input of $R_r$ and $R_s$ matrices can be removed to save memory bandwidth because of the fixed pattern that can be fused into the loop index. 
Custom code transformation that exploits the structure sparsity is conducted to optimize matrix multiplications, transforming multiplications to only load and store operations, sometimes with a small
number of additions.
\figref{fig:sr_reduction}(a) shows that all the multiplications and additions for MMM1/2 units are removed and \figref{fig:sr_reduction}(b) shows that only 6,960 (3.3\%) of the additions of the original implementation~\cite{moreno2020jedi} are required for the MMM3 unit in JEDI-net-30p models. There is a 96.7\% reduction in the number of iterations for all the MMM units, which significantly reduces the design latency.
\figref{fig:sr_reduction}(c) and (d) show the operations reduction in JEDI-net-50p models. 
%Besides, strength reduction also decreases the number of the total loop iterations to 2\% for all the MMM units, which largely reduces the design latency. 
Moreover, the run time of C synthesis using Vivado HLS is also reduced by over 3 times when compared with the HLS design without custom code transformation. 
%strength reduction. 


To achieve low latency and high throughput, the loops in each of the layers in the $f_R$, $f_O$, $\phi_O$ units are firstly fully unrolled. The proposed custom MMMs are applied with a column-major order data representation. The latency of our designs reduces from a few milliseconds to a few microseconds for both JEDI-net 30p and 50p models.
%, as shown in~\figref{fig:latency_reduction}. 
Based on these initial optimizations, the designs~\textbf{J1} and~\textbf{U1} are created for JEDI-net-30p and JEDI-net-50p respectively, as shown in~\tabref{table:cmp_u250}. They are used as the baseline designs in the comparison in the following sections. 
%The design~\textbf{J1} and~\textbf{U1} are used as the baseline designs that have initial parallelism parameters for JEDI-net-30p and JEDI-net-50p respectively, as shown in~\tabref{table:cmp_u250}.




\section{Introduction}

Graph neural networks (GNNs) have been explored and shown excellent performance for many fields including recommendation systems~\cite{ying2018graph, yang2019aligraph}, molecular property prediction~\cite{wu2018moleculenet}, and many high energy physics applications, such as jet tagging~\cite{moreno2020jedi}, charged particle tracking~\cite{ju2021performance,elabd2021graph}, and calorimeter energy measurements~\cite{qasim2019learning}.
Real-time data processing from high-energy proton collisions at the CERN Large Hadron Collider (LHC) is challenging since the particle detectors around the LHC ring produce hundreds of terabytes of data per second~\cite{coelho2021automatic, duarte2018fast} from collisions happening every 25 ns. 
In the next phase of the LHC, the upgraded High-Luminosity LHC (HL-LHC) experiments expect an explosion of data due to cutting edge detectors with improved resolution and increased area as well as volume.
The large data volumes produced from the detectors are reduced by a real-time processing system, known as the trigger, which keeps interesting collision events while discarding the others. 
The Level-1 Trigger~(L1T), using only FPGAs, requires processing latency of applications in $\mathcal{O}(1)\mu$s in the LHC~\cite{CERN2020L1T}. If algorithm latency exceeds this strict limit, valuable data and significant events are lost. 
 

Earlier trigger methodologies~\cite{cheatham2016atlas} relied solely on jet energy to make a decision. Recently, machine learning based strategies are being used for their superior accuracy. However, due to the low latency requirement, only uncomplicated Multi-Layer Perceptron (MLP) networks~\cite{coelho2021automatic, duarte2018fast} on FPGAs are introduced. High accuracy in the trigger is crucial to keep only the most interesting events while keeping the output bandwidth low~\cite{coelho2021automatic}. As a solution, the study in~\cite{moreno2020jedi} presents JEDI-net, a Graph Neural Network (GNN) based algorithm, that delivers state-of-the-art accuracy for particle identification. This development has led to a surge in the demand for GNNs in trigger systems.

However, GNNs require large amounts of computation and suffer from irregular memory accesses, leading to substantial inference latency. This hinders their effective deployment for real-time, ultra-low latency applications, such as the L1T system in a LHC experiment as suggested by Moreno et al.~\cite{moreno2020jedi}. 
Accelerating GNN inference using reconfigurable accelerators such as FPGAs is essential in the LHC since it enables sophisticated processing in real-time with superior accuracy. Nonetheless, most existing FPGA-based GNN accelerators employ a single-engine architecture with fixed hardware to sequentially process layers or sub-layers (blocks) like GPUs, and the networks are processed in a recurrent fashion~\cite{yan2020hygcn, liang2020engn, zhang2021boostgcn, lin2021gcn,lin2022hp,kang2022grow}. However, they are not efficient for GNN execution when handling small graphs that necessitate ultra-low latency and high throughput, such as in scientific applications for particle identification. Furthermore, none of them is designed to operate under a hard latency constraint in one microsecond ($\mathcal{O}(1)\mu$s). 

%a scenario with a hard constraint of latency in $\mathcal{O}(1)\mu$s. 

%are often designed using a single engine architecture with fixed hardware to process layers or sub-layers (blocks) repeatedly like GPUs, and the networks are processed in a recurrent fashion~\cite{yan2020hygcn, liang2020engn, zhang2021boostgcn, lin2021gcn,lin2022hp,kang2022grow}. However, they are not efficient for GNN execution when targeting small graphs with requirements of ultra-low latency and high throughput for scientific applications, such as particle identification. Also none of them targets a scenario with a hard constraint of latency in $\mathcal{O}(1)\mu$s. 


%But there are many challenges in developing an accelerator for GNNs, especially the one used in ultra low latency environment. GNNs usually suffers in irregular memory access
%This work proposes several optimizations to accelerate the GNN-based JEDI-net using high-level synthesis (HLS) on FPGAs. We also open-source the HLS templates of the graph neural network of JEDI-net for the community.  

%achieve a sub-microsecond latency. 

%In the trigger system, jet tagging is an important but challenging task. It identifies the decays of high-momentum heavy particles produced at the LHC and distinguishes them from ordinary jets which come from the hadronization of quarks and gluons. High accuracy in the trigger is crucial to keep only the most interesting events while keeping the output bandwidth low. 

%they cannot support low-latency and effective GNN execution when targeting small to medium GNN models with requirements of ultra low latency and ultra high throughput for scientific applications. 

This work proposes a custom Low Latency (LL)-GNN hardware architecture based on a layer-wise tailor-made pipeline with task-level parallelism to accelerate the GNNs for particle detectors. It uses the GNN-based JEDI-net algorithm as an end-to-end application. The layer-wise architecture has been used to speedup CNNs~\cite{blott2018finn, shen2017maximizing, zhang2020dnnexplorer} and RNNs~\cite{que2021accelerating}, but there remains a lack of focused research on accelerating GNNs.
%few studies focus on accelerating GNNs. 
To addresses the gap, this work introduces an outer-product based matrix-matrix multiplication (MMM) approach for calculating the GNN aggregation function, which is further enhanced by exploiting the structured adjacency matrix.
In addition, the proposed architecture adopts a column-major order instead of conventional row-major order for the data layout of intermediate results traversed along the hardware datapath, which avoids irregular memory access for intermediate results in GNNs. 
Moreover, this paper presents a custom code transformation for MMMs of GNN feature transformation based on the character of interaction-network based GNNs that utilize a fully connected graph as input. This approach avoids the costly matrix multiplications between the adjacency matrix and the input feature matrix, thereby enhancing computation efficiency. 
%It reduces the computational complexity and also avoids the irregular memory access of the sparse adjacency matrices since there is no need to fetch them. 
%resulting in improvement of throughput as well as reduction in latency. 

%The number of its columns is nearly the square of the number of input particles. 
%We also utilize scratchpad memories to store these
%To deal with the irregular memory access, we utilize a scratchpad memory to store the matrices that need random access.

%which inputs and outputs the data in a column-major order to increase the data spatial locality and alleviate irregular memory access to reduce the design latency. 
%Additionally, it is further enhanced by exploiting the structured sparsity of the of the adjacency matrix.  
%It not only avoids expensive multiplication and involves just a few additions, but also avoids the input of the adjacency matrix to remove irregular memory access and save memory bandwidth. 
%Moreover, this work introduces a two-level parallelism scheme which explores potential design parallelism. 
%this work balances the IIs of sub-layers by hardware resource reallocation to achieve low IIs with a given FPGA. 
%Furthermore, design space exploration is performed to identify the appropriate parallelism parameters. Finally, a fine-tuning step is conducted to find the design with not only low II but also low end-to-end latency. 

%Most of them can only support layer-wise GNNs without custom architecture, e.g., skip-connection. 
%Second, they rely on CPUs as a HOST for control, or even partially computation. In \cite{xxx}, xxx computation is done in CPUs. 
%They will degrade the accelerator performance and efficiency because of the lack of fine-grained customizability. 
%splits the whole GNN model into several sub-layers and 
 
%Besides, our previous designs~\cite{que2022aicas, que2022optimizing} prioritize to optimize initiation interval. It may not lead to a optimal end-to-end latency which is key for designs running in the CERN L1T system. 

Furthermore, instead of running GNNs in a coarse-grained pipeline as shown in our prior work~\cite{que2022aicas, que2022optimizing}, this work fuses sub-layers as much as possible, transforming multiple coarse-grained pipeline stages into a singular stage with a fine-grained pipeline inside. 
The fusion eliminates unnecessary handshake acknowledgments and dual buffers between coarse-grained pipeline stages, effectively reducing end-to-end latency. 
To further optimize latency, we introduce a Finite State Machine (FSM)-based code structure to handle any imperfect loops that may emerge after fusion.
%It is the first time that the GNNs of JEDI-net can run in less than $1\mu$s on FPGAs. 
Finally, we present a GNN-specific algorithmic-hardware co-design approach to optimize the algorithm and hardware simultaneously, and to explore the optimal configuration to enhance overall performance. Our LL-GNN design successfully achieves a sub-microsecond latency, which makes the algorithm compatible with the HL-LHC conditions where there is a hard ultra-low latency constraint, while also enabling improved accuracy.

To the best of our knowledge, this is the first FPGA-based design of GNNs with a latency in $\mathcal{O}(1)\mu$s for particle identification for the detectors at the CERN HL-LHC experiments.
%he next phase of the LHC (High-Luminosity LHC) 
%In the next phase of the LHC (the High-Luminosity LHC), the upgraded experiments would expect an explosion of data due to cutting edge detectors with improved resolution and increased area as well as volume. 
%This work would help to improve the next-generation trigger system, enabling more powerful algorithms to filter the right experimental data more accurately and efficiently. 
This work would help to improve next-generation trigger systems, enabling powerful algorithms to process experimental data effectively. 


%This work adopts a layer-wise tailor-made pipeline architecture mapping on-chip, which is flexible and able to take full advantage of the customizability of FPGAs. First, this work splits the whole GNN model into several sub-layers and conduct dedicated optimizations to each sub-layer. Second, instead of running these sub-layers in a coarse-grained pipeline as shown in our previous work~\cite{que2022aicas, que2022optimizing}, this work fusions sub-layers as many as possible, converting the design from a coarse-grained pipeline to a fine-grained pipeline to avoid extra acknowledgments between units, result in ultra low end-to-end (E2E) latency. It is the first time that this GNN can run on an FPGA in less than $1\mu$s. 
%And all the sub-layers are mapped on-chip and run in a pipeline with dedicated optimization for each of them to further increase the design throughput. 

%and a latency below 2$\mu$s. 

%With both of the above optimizations, our FPGA implementation of JEDI-net achieves sub-microsecond initiation interval (II), which makes the model deployable at the collider trigger system that has strict latency constraints, while enabling the system to benefit from improved accuracy.


%we propose custom strength reduction for matrix operations based on the characters of the JEDI-net, which avoids the expensive matrix multiplications of the adjacency matrix with the input feature matrix. It largely reduces the computation cost of JEDI-net and boosts the design throughput since the adjacency matrix is very large and matrix multiplication is costly. 
%The number of its columns is nearly the square of the number of input particles. 
%Second, we propose to adopt column-major order instead of the conventional row-major order for the data layout of the intermediate results traversed along the hardware datapath, which benefits the computation of JEDI-net. 
%Moreover, we optimize the JEDI-net aggregation function computation using an outer-product based matrix multiplication which inputs and outputs the data in a column-major order to increase the data spatial locality and reduce the design latency. 
%It enables a coarse grained pipeline with a low initiation interval to improve the design throughput.  
%With both of the above optimizations, our FPGA implementation of JEDI-net achieves sub-microsecond initiation interval (II), which makes the model deployable at the collider trigger system that has strict latency constraints, while enabling the system to benefit from improved accuracy.


%which could enable the inclusion of jet identifying GNNs at the trigger level for LHC experiments 

%identifies all-hadronic decays of high-momentum heavy particles produced at the LHC and distinguish them from ordinary jets originating from the hadronization of quarks and gluons.

%\iffalse

%\fi

We make the following contributions in this paper:
\begin{itemize}

%\item A custom strength reduction for matrix multiplications in the interaction-network based GNNS with an input of fully connected graphs, which exploits sparsity patterns and binary adjacency matrices as well as avoiding irregular memory accesses, leading to high hardware efficiency and low design latency. 

%\item An outer-product based matrix multiplication approach combined with custom strength reduction as well as column-major order data layout to increase hardware efficiency and reduce design latency. 

%\item A low latency pipeline design for GNNs combining the above novel hardware optimizations and sub-layer fusion as well as a GNN-specific algorithmic and hardware co-optimizations approach, resulting in sub-microsecond design latency. 


\item A low latency layer-wise hardware architecture for GNNs with many novel design optimizations, including outer-product based matrix multiplication, column-major order, custom code transformation and the fusion of sub-layers as well as a GNN-specific algorithm and hardware co-optimization approach, resulting in sub-microsecond latency and high hardware efficiency.  

%\item A low latency pipeline design for GNNs with several hardware optimizations, including custom strength reduction, column-major order and outer-product based matrix multiplication as well as sub-layer fusion, resulting in sub-microsecond design latency and high hardware efficiency.  

%novel column-major order based data layout to increase design throughput and reduce design latency. 
%\item A custom strength reduction for matrix multiplications in the GNN-based JEDI-net, which exploits sparsity patterns and binary adjacency matrices to increase hardware efficiency while reducing latency. 

%\item An outer-product based matrix multiplication approach combined with custom strength reduction as well as column-major order data layout, resulting in high hardware efficiency and low design latency. 

%\item \textcolor{red}{TODO}minimise and balance the initiation interval 
%\item A custom strength reduction for matrix multiplications for the GNN-based JEDI-net, which exploits sparsity patterns and binary adjacency matrices to increase hardware efficiency while reducing latency. 

%\item A low latency coarse-grained pipeline design for JEDI-net with novel column-major order data layout to increase design throughput and reduce the design latency for jet identification. 
%\item The first FPGA-based design of GNNs with a latency in $\mathcal{O}(1)\mu$s for particle identification for the detectors at the CERN HL-LHC experiments.

\item A scalable, efficient open-source template\footnote{https://github.com/walkieq/GNN-JEDInet-FPGA} for GNN-based JEDI-net, which enables the generation of low-latency FPGA designs with efficient resource utilization leveraging high-level synthesis (HLS) tools. 

\item A comprehensive evaluation of the proposed method and hardware architecture. 


\end{itemize}

While our research primarily utilizes GNN-based JEDI-net to illustrate our hardware architecture and development approach, the proposed optimizations could be applied to other GNN networks with small graphs for applications beyond particle identification. Moreover, the techniques devised for low latency optimization can benefit numerous other applications on FPGAs, especially those that require real-time processing. 

%This section introduces several optimizations to accelerate the GNN for JEDI-net. Although this work focuses on the architecture of JEDI-net for jet tagging, the proposed techniques could be adapted to optimize other GNN-based networks with applications beyond jet tagging. 

%The specific RNN layered structure and coefficients are LIGO specific, but the need for low latency would benefit many other applications, especially those requiring real-time response, e.g., low latency would benefit the Large Hadron Collider (LHC) physics~\cite{duarte2018fast}, adaptive radiotherapy~\cite{thorwarth2021technical} and electronic trading~\cite{denholm2014low}. The proposed techniques can be adapted to address these other applications. 

%[18] achieves both microsecond level initiation interval and latency

\subsubsection*{Relationship to Prior Publications}
This paper expands on our previous work~\cite{que2022aicas, que2022optimizing} which focuses on hardware optimizations and targets low initiation interval, but still suffer from high latency. 
%This work addresses two limitations of the prior work. 
First, we focus on optimizing end-to-end latency while prior work concerns with initiation interval. 
Our new approach fuses together as many coarse-grained pipeline stages as possible into a single fine-grained pipeline stage, resulting in low latency designs. 
Second, we cover co-optimization of algorithm and hardware, while prior work concerns only with hardware optimizations. 
%In addition, a GNN-specific co-design approach is proposed to optimize the algorithm and hardware simultaneously. 
This work explores the design performance trade-off under both user-defined algorithm and hardware constraints, such as achieving the highest accuracy with a latency requirement of less than 1$\mu$s on a given FPGA. 
The optimized design provides a significant reduction in end-to-end latency, achieving speedups of 6.51 to 16.7 times with improved model accuracy compared to our previous work~\cite{que2022aicas, que2022optimizing}. 
Our novel architecture in this work is the first to support GNNs of JEDI-net to run in less than 1$\mu$s on FPGAs. To facilitate the deployment of these optimizations, we provide an open-source template for generating low-latency FPGA implementations of GNN-based JEDI-net with efficient resource utilizations.
%In addition, it is the first time that the GNNs of JEDI-net can run in less than 1$\mu$s on FPGAs, which was not achieved in our previous two articles. 
%These novel optimizations, combining the ones in our previous work, lead to sub-microsecond design latency, which makes the algorithm compatible with the CERN HL-LHC where there is a strict latency constraint of $\mathcal{O}(1)\mu$s. 

%Firstly, they focus on initiation intervals rather than end-to-end latency. Secondly, they only cover hardware optimizations but do not consider co-optimization of algorithmic and hardware. 


%This work addresses a limitation in our previous work, which does not cover co-design of algorithmic and hardware optimizations.  This limitation results in a sub-optimal design with large latency, which hinders the deployment of GNNs in the CERN LHC. 
%This work presents a GNN-specific co-design approach to optimize the algorithm and hardware simultaneously. Our approach can explore the design performance trade-off under both user-defined algorithm and hardware constraints, e.g., the highest accuracy with a latency requirement of less than 1$\mu$s on a given FPGA.
%and find the optimal design with both accepted model accuracy and hardware latency on a given FPGA. 
%a GNN-specific co-design approach to optimize the algorithm and hardware simultaneously.
%In addition, a new low latency hardware architecture with sub-layer fusion is proposed, which targets end-to-end latency reduction instead of initiation interval. It fuses several coarse-grained pipeline stages into a single stage with fine-grained pipeline inside using an FSM-based code transformation, resulting in low latency designs. 
%The new optimizations proposed allow us to obtain a significant reduction in end-to-end latency over our previous work~\cite{que2022aicas, que2022optimizing}. 
%6.51 to 16.7 times lower end-to-end latency over our previous work~\cite{que2022aicas, que2022optimizing}. 
%a significant reduction in end-to-end latency over our previous work~\cite{que2022aicas, que2022optimizing}. 
%Compared to our previous FPGA implementations, this work achieves 6.51 to 16.7 times lower latency.
%These novel optimizations, combining the ones in our previous work, lead to sub-microsecond design latency, which makes the algorithm compatible with the CERN HL-LHC where there is a strict latency constraint of $\mathcal{O}(1)\mu$s. 

%This paper adds the design of multiple sub-accelerator cores for spatial co-execution of RNNs in~\secref{subsec:multicore}.  \secref{subsec:system}-\ref{subsec:system_others} describe a revised hardware architecture, and~\secref{subsec:to_gpu}-\ref{subsec:to_fpga} contain new evaluation results. 


\begin{figure}
\begin{center}
\includegraphics[width=0.7\linewidth]{img/accuracy_t01.pdf}
\end{center}
   \caption{
   %The accuracy of JEDI-net 50p model for a range of bit widths.
   Model accuracy of JEDI-net 50p network under different datapath bitwidth configurations. The x-axis represents the total number of bits, while the different colored lines with dots represent varying numbers of integer bits. The line without dots shows the model accuracy using 32-bit floating-point (FP32) representation.  
   %The accuracy of the model is analyzed under different bitwidth configurations to determine the optimal bitwidth for balancing accuracy and computational complexity.}
   }
\label{fig:accuracy}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=0.6\linewidth]{img/auc_10k_m03.pdf}
\end{center}
   \caption{The AUCs of five jet taggers.}
\label{fig:auc_10k}
\end{figure}

